Graviton scattering amplitudes in first quantisation

We give a pedagogical review to alternative, first quantised approaches to calculating graviton scattering amplitudes, giving an introduction to string inspired approaches and presenting more recent work based on the worldline formalism of quantum field theory that is motivated by these historic results. We describe how these first quantised techniques can greatly simplify the determination of such amplitudes, in particular reducing the number of Feynman-like diagrams that enter the computation and leading to compact results.

==> Gravitons <==
SyncTeX Version:1
Input:1:C:\Users\eddy_\Dropbox\University\Mexico\Presentations\2021 08 DPyC\Proceedings\Plantilla-rmf\Research-Education-ingles.tex
Input:2:C:\Users\eddy_\Dropbox\University\Mexico\Presentations\2021 08 DPyC\Proceedings\Plantilla-rmf\rmf-d.cls
Input:3:C:\Program Files\MiKTeX\tex\latex\base\leqno.clo
Input:4:C:\Program Files\MiKTeX\tex\latex\base\size10.clo
Input:5:C:\Users\eddy_\Dropbox\University\Mexico\Presentations\2021 08 DPyC\Proceedings\Plantilla-rmf\nopageno.sty
Input:6:C:\Users\eddy_\Dropbox\University\Mexico\Presentations\2021 08 DPyC\Proceedings\Plantilla-rmf\rmfbib.sty
Input:7:C:\Program Files\MiKTeX\tex\latex\tools\multicol.sty
Input:8:C:\Program Files\MiKTeX\tex\latex\psnfss\times.sty
Input:9:C:\Program Files\MiKTeX\tex\latex\epsf\epsf.sty
Input:10:C:\Program Files\MiKTeX\tex\latex\amsmath\amsmath.sty
Input:11:C:\Program Files\MiKTeX\tex\latex\amsmath\amstext.sty
Input:12:C:\Program Files\MiKTeX\tex\latex\amsmath\amsgen.sty
Input:13:C:\Program Files\MiKTeX\tex\latex\amsmath\amsbsy.sty
Input:14:C:\Program Files\MiKTeX\tex\latex\amsmath\amsopn.sty
Input:15:C:\Program Files\MiKTeX\tex\latex\amsfonts\amssymb.sty
Input:16:C:\Program Files\MiKTeX\tex\latex\amsfonts\amsfonts.sty
Input:17:C:\Program Files\MiKTeX\tex\latex\cite\cite.sty
Input:18:C:\Program Files\MiKTeX\tex\latex\base\inputenc.sty
Input:19:C:\Program Files\MiKTeX\tex\latex\base\latin1.def
Input:20:C:\Users\eddy_\Dropbox\University\Mexico\Presentations\2021 08 DPyC\Proceedings\Plantilla-rmf\caption2.sty
Input:21:C:\Program Files\MiKTeX\tex\latex\graphics\graphics.sty
Input:22:C:\Program Files\MiKTeX\tex\latex\graphics\trig.sty
Input:23:C:\Program Files\MiKTeX\tex\latex\graphics-cfg\graphics.cfg
Input:24:C:\Program Files\MiKTeX\tex\latex\graphics-def\pdftex.def
Input:25:C:\Program Files\MiKTeX\tex\latex\psnfss\ot1ptm.fd
Input:26:C:\Program Files\MiKTeX\tex\latex\l3backend\l3backend-pdftex.def
Input:27:C:\Users\eddy_\Dropbox\University\Mexico\Presentations\2021 08 DPyC\Proceedings\Plantilla-rmf\Research-Education-ingles.aux
Input:28:C:\Program Files\MiKTeX\tex\latex\amsfonts\umsa.fd
Input:29:C:\Program Files\MiKTeX\tex\latex\amsfonts\umsb.fd
Input:30:C:\Program Files\MiKTeX\tex\context\base\mkii\supp-pdf.mkii
Input:31:C:\Program Files\MiKTeX\tex\latex\epstopdf-pkg\epstopdf-base.sty
Input:32:C:\Program Files\MiKTeX\tex\latex\00miktex\epstopdf-sys.cfg
Output:pdf
Magnification:1000
Unit:1
X Offset:0
Y Offset:0
Content:
!2444
{1
[1,90:4736286,49947279:32556487,47579136,0
(1,90:4736286,2368143:0,0,0
[1,90:0,2368143:0,0,0
(1,90:0,-2368143:0,0,0
g1,90:0,-2368143
)
]
)
[1,90:4262629,49947279:33030144,47579136,0
[1,90:4262629,3154575:33030144,786432,0
(1,90:4262629,3154575:33030144,0,0
h1,90:4262629,3154575:33030144,0,0
)
]
[1,90:4262629,47981199:33030144,44040192,0
(1,41:4262629,3023503:33030144,450225,9168
g1,41:4262629,3023503
g1,41:4426469,3023503
x1,41:5154565,3023503
x1,41:6376131,3023503
g1,41:6539971,3023503
x1,41:7413555,3023503
x1,41:9114202,3023503
g1,41:9278042,3023503
x1,41:9896698,3023503
g1,41:10060538,3023503
x1,41:10424914,3023503
(1,41:10406889,3020226:218232,446948,0
x1,41:10625121,3020226
)
x1,41:11626160,3023503
g1,41:11790000,3023503
k1,41:32961526,3023503:21171526
x1,41:35654373,3023503
g1,41:35818213,3023503
x1,41:37128933,3023503
g1,41:37292773,3023503
g1,41:37292773,3023503
)
(1,41:4262629,4871611:33030144,650217,192038
k1,41:10303030,4871611:6040401
h1,41:10303030,4871611:0,0,0
x1,41:11928097,4871611
x1,41:13949521,4871611
g1,41:14185450,4871611
x1,41:18168833,4871611
g1,41:18404762,4871611
x1,41:22861881,4871611
g1,41:23097810,4871611
x1,41:23884855,4871611
g1,41:24120784,4871611
x1,41:25745841,4871611
g1,41:25981770,4871611
x1,41:31016444,4871611
g1,41:31252373,4871611
g1,41:31252373,4871611
k1,41:37292773,4871611:6040400
)
(1,41:4262629,6326503:33030144,446948,9168
k1,41:18442023,6326503:14179394
h1,41:18442023,6326503:0,0,0
x1,41:20043694,6326503
g1,41:20207534,6326503
x1,41:20571910,6326503
x1,41:20663005,6326503
g1,41:20826845,6326503
x1,41:22028117,6326503
x1,41:23113380,6326503
g1,41:23113380,6326503
k1,41:37292774,6326503:14179394
)
(1,41:4262629,7112935:33030144,448587,135328
k1,41:17761759,7112935:13499130
h1,41:17761759,7112935:0,0,0
x1,41:19910006,7112935
x1,41:22855172,7112935
x1,41:23793642,7112935
g1,41:23793642,7112935
k1,41:37292772,7112935:13499130
)
(1,48:4262629,11208935:33030144,402253,127692
h1,46:4262629,11208935:0,0,0
x1,46:4819419,11208935
x1,46:5034115,11208935
k1,46:5146203,11208935:112088
x1,46:5605080,11208935
x1,46:5885246,11208935
x1,46:6138282,11208935
k1,46:6250370,11208935:112088
x1,46:6512248,11208935
k1,46:6624336,11208935:112088
x1,46:9474338,11208935
k1,46:9586426,11208935:112088
x1,46:10044713,11208935
x1,46:10750722,11208935
x1,46:11161827,11208935
k1,46:11273914,11208935:112087
x1,46:11732791,11208935
k1,46:11844879,11208935:112088
x1,46:13777694,11208935
x1,46:14057860,11208935
x1,46:14458352,11208935
k1,46:14577514,11208935:119162
x1,46:15495261,11208935
k1,46:15607349,11208935:112088
x1,46:17868118,11208935
k1,46:17980206,11208935:112088
x1,46:20633210,11208935
k1,46:20745298,11208935:112088
x1,46:21204175,11208935
k1,46:21316263,11208935:112088
x1,46:23904371,11208935
k1,46:24016459,11208935:112088
x1,46:24769658,11208935
x1,46:25970530,11208935
k1,46:26082617,11208935:112087
x1,46:28375814,11208935
k1,46:28487902,11208935:112088
x1,46:31224057,11208935
k1,46:31343219,11208935:119162
x1,46:32129452,11208935
x1,46:33628188,11208935
k1,46:33740276,11208935:112088
x1,46:34297066,11208935
k1,46:34409154,11208935:112088
x1,46:37292773,11208935
k1,46:37292773,11208935:0
)
(1,48:4262629,11995367:33030144,402253,127692
x1,48:4721506,11995367
k1,46:4894194,11995367:172688
x1,46:6237792,11995367
k1,46:6410480,11995367:172688
x1,46:8310868,11995367
k1,46:8483556,11995367:172688
x1,46:11136560,11995367
k1,46:11309248,11995367:172688
x1,46:12160950,11995367
k1,46:12333638,11995367:172688
x1,46:14790816,11995367
k1,46:14963504,11995367:172688
x1,46:16175580,11995367
k1,46:16348268,11995367:172688
x1,46:17789188,11995367
k1,46:17961876,11995367:172688
x1,46:18387727,11995367
x1,46:19168062,11995367
k1,46:19340750,11995367:172688
x1,46:20683765,11995367
k1,46:20856453,11995367:172688
x1,46:21446277,11995367
k1,46:21618966,11995367:172689
x1,46:22339721,11995367
k1,46:22512409,11995367:172688
x1,46:22938260,11995367
x1,46:24767280,11995367
k1,46:24939968,11995367:172688
x1,46:27364695,11995367
k1,46:27537383,11995367:172688
x1,46:28028704,11995367
k1,46:28201392,11995367:172688
x1,46:30265760,11995367
k1,46:30438448,11995367:172688
x1,46:31487141,11995367
k1,46:31659829,11995367:172688
x1,46:33166817,11995367
k1,46:33339505,11995367:172688
x1,46:34224225,11995367
k1,46:34396913,11995367:172688
x1,46:34790313,11995367
k1,46:34963001,11995367:172688
x1,46:36044720,11995367
x1,46:36324886,11995367
x1,46:37292773,11995367
k1,46:37292773,11995367:0
)
(1,48:4262629,12781799:33030144,402253,127692
x1,48:4852453,12781799
k1,46:5043755,12781799:191302
x1,46:6255823,12781799
k1,46:6447125,12781799:191302
x1,46:8216566,12781799
k1,46:8407868,12781799:191302
x1,46:10095323,12781799
k1,46:10409705,12781799:314382
x1,46:10966495,12781799
x1,46:11181191,12781799
k1,46:11372493,12781799:191302
x1,46:13337760,12781799
k1,46:13529062,12781799:191302
x1,46:14118886,12781799
x1,46:14529991,12781799
k1,46:14721292,12781799:191301
x1,46:15933360,12781799
k1,46:16124662,12781799:191302
x1,46:17042409,12781799
k1,46:17233711,12781799:191302
x1,46:19494480,12781799
k1,46:19685782,12781799:191302
x1,46:22208429,12781799
k1,46:22399731,12781799:191302
x1,46:23218399,12781799
k1,46:23409701,12781799:191302
x1,46:25047620,12781799
k1,46:25238922,12781799:191302
x1,46:27205362,12781799
k1,46:27396664,12781799:191302
x1,46:28117419,12781799
k1,46:28308721,12781799:191302
x1,46:31585149,12781799
k1,46:31776451,12781799:191302
x1,46:32267772,12781799
k1,46:32459074,12781799:191302
x1,46:33540211,12781799
k1,46:33731513,12781799:191302
x1,46:36467668,12781799
k1,46:36669931,12781799:202263
x1,46:37292773,12781799
k1,46:37292773,12781799:0
)
(1,48:4262629,13568231:33030144,402253,127692
x1,48:6522800,13568231
g1,46:6670256,13568231
x1,46:8734034,13568231
g1,46:8881490,13568231
x1,46:9602245,13568231
g1,46:9749701,13568231
x1,46:11551601,13568231
g1,46:11699057,13568231
x1,46:12190378,13568231
g1,46:12337834,13568231
x1,46:12927650,13568231
x1,46:14720708,13568231
x1,46:15343550,13568231
x1,46:15599530,13568231
g1,46:15746986,13568231
x1,46:17909252,13568231
g1,46:18056708,13568231
x1,46:18941428,13568231
g1,46:19088884,13568231
x1,46:20267926,13568231
g1,46:20415382,13568231
x1,46:21136137,13568231
g1,46:21283593,13568231
x1,46:24380137,13568231
g1,46:24562981,13568231
g1,46:24562981,13568231
k1,48:24562981,13568231:0
k1,48:37292773,13568231:12729792
g1,48:37292773,13568231
)
(1,50:4262629,15337703:33030144,403728,127692
h1,50:4262629,15337703:0,0,0
x1,50:4656037,15337703
x1,50:4897272,15337703
x1,50:6059214,15337703
x1,50:6758146,15337703
g1,50:6940990,15337703
g1,50:7123834,15337703
x1,50:9319141,15337703
g1,50:9466597,15337703
x1,50:10679255,15337703
g1,50:10826711,15337703
x1,50:12530115,15337703
x1,50:12639238,15337703
g1,50:12786694,15337703
x1,50:13670832,15337703
x1,50:15248595,15337703
g1,50:15396051,15337703
x1,50:17787751,15337703
g1,50:17935207,15337703
x1,50:20687879,15337703
g1,50:20835335,15337703
k1,50:37292773,15337703:16457438
g1,50:37292773,15337703
)
(1,87:4262629,41093349:33030144,25100286,141880
[1,87:4262629,41093349:15925248,25100286,0
(1,57:4262629,16648423:15925248,541848,11006
(1,57:4262629,16648423:1376256,541848,11006
g1,57:4262629,16648423
x1,57:4852453,16648423
g1,57:5638885,16648423
)
x1,57:6993100,16648423
x1,57:9906804,16648423
k1,57:20187877,16648423:10281073
g1,57:20187877,16648423
)
(1,60:4262629,18024677:15925248,446948,141880
x1,60:5281709,18024677
k1,59:5478709,18024677:197000
x1,59:6534476,18024677
x1,59:7699044,18024677
k1,59:7896044,18024677:197000
x1,59:8514700,18024677
x1,59:10297924,18024677
k1,59:10494924,18024677:197000
x1,59:11004787,18024677
k1,59:11201788,18024677:197001
x1,59:11820444,18024677
x1,59:12548539,18024677
x1,59:13385427,18024677
x1,59:13749793,18024677
x1,59:14061089,18024677
x1,59:14342241,18024677
k1,59:14539241,18024677:197000
x1,59:15813257,18024677
x1,59:16832983,18024677
k1,59:17029983,18024677:197000
x1,59:18195198,18024677
k1,59:18392198,18024677:197000
x1,59:19193037,18024677
x1,59:20066629,18024677
x1,59:20187877,18024677
k1,59:20187877,18024677:0
)
(1,60:4262629,18811109:15925248,446948,141880
x1,60:5754869,18811109
k1,59:6032667,18811109:277798
x1,59:6688027,18811109
k1,59:6965825,18811109:277798
x1,59:7766664,18811109
k1,59:8044462,18811109:277798
x1,59:8699814,18811109
x1,59:9527533,18811109
x1,59:10838235,18811109
k1,59:11116034,18811109:277799
x1,59:11625897,18811109
x1,59:11916873,18811109
x1,59:13263624,18811109
k1,59:13541422,18811109:277798
x1,59:13832398,18811109
x1,59:14150254,18811109
x1,59:15096590,18811109
x1,59:16189061,18811109
k1,59:16466859,18811109:277798
x1,59:17449881,18811109
k1,59:17727679,18811109:277798
x1,59:18055359,18811109
x1,59:18273591,18811109
x1,59:18589479,18811109
x1,59:19204862,18811109
x1,59:20187877,18811109
k1,59:20187877,18811109:0
)
(1,60:4262629,19597541:15925248,446948,141880
x1,60:5208965,19597541
x1,60:5791563,19597541
x1,60:6119243,19597541
x1,60:6433819,19597541
x1,60:7708473,19597541
k1,59:7886948,19597541:178475
x1,59:8468900,19597541
x1,59:9633468,19597541
x1,59:10471011,19597541
k1,59:10649486,19597541:178475
x1,59:11159349,19597541
k1,59:11337824,19597541:178475
x1,59:12138663,19597541
k1,59:12317139,19597541:178476
x1,59:13482362,19597541
x1,59:14319250,19597541
k1,59:14497725,19597541:178475
x1,59:15043637,19597541
k1,59:15222112,19597541:178475
x1,59:15950207,19597541
x1,59:17369693,19597541
k1,59:17548168,19597541:178475
x1,59:19132159,19597541
k1,59:19314293,19597541:182134
x1,59:20187877,19597541
k1,59:20187877,19597541:0
)
(1,60:4262629,20383973:15925248,446948,141880
x1,60:5682124,20383973
k1,59:5918301,20383973:236177
x1,59:7702180,20383973
k1,59:7938356,20383973:236176
x1,59:8811940,20383973
x1,59:9903748,20383973
x1,59:10631843,20383973
k1,59:10868020,20383973:236177
x1,59:11560066,20383973
k1,59:11796243,20383973:236177
x1,59:12269402,20383973
x1,59:12779265,20383973
x1,59:13236049,20383973
x1,59:14073592,20383973
k1,59:14309768,20383973:236176
x1,59:15693223,20383973
x1,59:18095741,20383973
k1,59:18331918,20383973:236177
x1,59:19168806,20383973
x1,59:19969645,20383973
x1,59:20187877,20383973
k1,60:20187877,20383973:0
)
(1,60:4262629,21170405:15925248,446948,141880
x1,60:5537283,21170405
k1,59:5813656,21170405:276373
x1,59:6577800,21170405
k1,59:6854173,21170405:276373
x1,59:7873236,21170405
x1,59:8346395,21170405
x1,59:9402170,21170405
k1,59:9678543,21170405:276373
x1,59:10552135,21170405
x1,59:12189847,21170405
k1,59:12466220,21170405:276373
x1,59:12648403,21170405
x1,59:12976083,21170405
x1,59:13277554,21170405
x1,59:14101993,21170405
x1,59:14939536,21170405
k1,59:15215909,21170405:276373
x1,59:16089501,21170405
x1,59:16708157,21170405
x1,59:17836676,21170405
x1,59:18492018,21170405
k1,59:18768391,21170405:276373
x1,59:19387047,21170405
x1,59:19969645,21170405
x1,59:20187877,21170405
k1,60:20187877,21170405:0
)
(1,60:4262629,21956837:15925248,446948,141880
x1,60:5445532,21956837
k1,59:5636720,21956837:191188
x1,59:6437568,21956837
x1,59:6894352,21956837
x1,59:7185328,21956837
x1,59:7496624,21956837
x1,59:7996008,21956837
x1,59:8133639,21956837
k1,59:8268743,21956837:135104
x1,59:8559719,21956837
x1,59:9962822,21956837
k1,59:10090743,21956837:127921
x1,59:10600606,21956837
k1,59:10728527,21956837:127921
x1,59:11966495,21956837
k1,59:12094416,21956837:127921
x1,59:12858551,21956837
x1,59:13477207,21956837
x1,59:13950366,21956837
x1,59:15225020,21956837
k1,59:15352941,21956837:127921
x1,59:15862804,21956837
k1,59:15990725,21956837:127921
x1,59:16281701,21956837
x1,59:16592997,21956837
x1,59:17092381,21956837
k1,59:17220302,21956837:127921
x1,59:18894733,21956837
k1,59:19022654,21956837:127921
x1,59:20187877,21956837
k1,59:20187877,21956837:0
)
(1,60:4262629,22743269:15925248,446948,141880
x1,60:4590309,22743269
x1,60:5900357,22743269
k1,59:6058610,22743269:158253
x1,59:6858794,22743269
k1,59:7017047,22743269:158253
x1,59:7927335,22743269
x1,59:8910357,22743269
k1,59:9068611,22743269:158254
x1,59:10197130,22743269
x1,59:10889176,22743269
x1,59:12271967,22743269
k1,59:12430220,22743269:158253
x1,59:13085580,22743269
k1,59:13243833,22743269:158253
x1,59:14044672,22743269
k1,59:14202925,22743269:158253
x1,59:14421157,22743269
x1,59:14996556,22743269
x1,59:15506419,22743269
x1,59:16379993,22743269
k1,59:16538247,22743269:158254
x1,59:17411839,22743269
x1,59:18378486,22743269
k1,59:18536739,22743269:158253
x1,59:19228785,22743269
k1,59:19387038,22743269:158253
x1,59:20187877,22743269
k1,59:20187877,22743269:0
)
(1,60:4262629,23529701:15925248,446948,141880
x1,60:5427852,23529701
x1,60:6264740,23529701
k1,59:6501099,23529701:236359
x1,59:7047011,23529701
k1,59:7283371,23529701:236360
x1,59:7793234,23529701
x1,59:8084210,23529701
x1,59:9685889,23529701
k1,59:9922248,23529701:236359
x1,59:10868584,23529701
k1,59:11104944,23529701:236360
x1,59:11905783,23529701
k1,59:12142142,23529701:236359
x1,59:12652005,23529701
x1,59:13998093,23529701
x1,59:14835636,23529701
k1,59:15071995,23529701:236359
x1,59:15581858,23529701
x1,59:16148082,23529701
x1,59:17458784,23529701
k1,59:17695144,23529701:236360
x1,59:18387190,23529701
k1,59:18623549,23529701:236359
x1,59:19205501,23529701
x1,59:19969645,23529701
x1,59:20187877,23529701
k1,60:20187877,23529701:0
)
(1,60:4262629,24316133:15925248,446948,141880
x1,60:5100172,24316133
k1,59:5278176,24316133:178004
x1,59:6115719,24316133
k1,59:6293723,24316133:178004
x1,59:7094562,24316133
k1,59:7272566,24316133:178004
x1,59:7781774,24316133
x1,59:8728748,24316133
x1,59:9566291,24316133
k1,59:9744295,24316133:178004
x1,59:11346619,24316133
x1,59:14550631,24316133
k1,59:14728635,24316133:178004
x1,59:15238498,24316133
x1,59:15420681,24316133
x1,59:15711657,24316133
x1,59:16975832,24316133
k1,59:17153836,24316133:178004
x1,59:17481516,24316133
x1,59:17799372,24316133
x1,59:18298756,24316133
k1,59:18476760,24316133:178004
x1,59:18986623,24316133
x1,59:20187877,24316133
k1,59:20187877,24316133:0
)
(1,60:4262629,25102565:15925248,446948,141880
x1,60:5100172,25102565
x1,60:6865690,25102565
k1,59:7222266,25102565:356576
x1,59:7986410,25102565
x1,59:9224360,25102565
k1,59:9439339,25102565:214979
x1,59:10386313,25102565
k1,59:10601292,25102565:214979
x1,59:11565971,25102565
k1,59:11793734,25102565:227763
x1,59:12302942,25102565
x1,59:13249916,25102565
x1,59:14087459,25102565
k1,59:14302437,25102565:214978
x1,59:15103276,25102565
x1,59:15795322,25102565
x1,59:17178769,25102565
k1,59:17393748,25102565:214979
x1,59:17939660,25102565
x1,59:18904339,25102565
k1,59:19132102,25102565:227763
x1,59:20187877,25102565
k1,59:20187877,25102565:0
)
(1,60:4262629,25888997:15925248,446948,141880
x1,60:5100172,25888997
k1,59:5271408,25888997:171236
x1,59:5781271,25888997
k1,59:5952507,25888997:171236
x1,59:6571163,25888997
k1,59:6742400,25888997:171237
x1,59:8198599,25888997
k1,59:8369835,25888997:171236
x1,59:9316809,25888997
x1,59:10335880,25888997
k1,59:10507116,25888997:171236
x1,59:11635635,25888997
k1,59:11806872,25888997:171237
x1,59:12316735,25888997
x1,59:12789894,25888997
x1,59:13808965,25888997
x1,59:14318828,25888997
x1,59:15082963,25888997
k1,59:15254199,25888997:171236
x1,59:16018334,25888997
x1,59:16636990,25888997
x1,59:17110149,25888997
x1,59:18384803,25888997
k1,59:18556039,25888997:171236
x1,59:19029207,25888997
x1,59:20187877,25888997
k1,59:20187877,25888997:0
)
(1,60:4262629,26675429:15925248,446948,141880
x1,60:5609372,26675429
k1,59:5746286,26675429:136914
x1,59:6256149,26675429
k1,59:6393064,26675429:136915
x1,59:7011720,26675429
x1,59:7667062,26675429
x1,59:7849245,26675429
x1,59:8941060,26675429
k1,59:9077974,26675429:136914
x1,59:10024310,26675429
k1,59:10161224,26675429:136914
x1,59:10707136,26675429
x1,59:11507975,26675429
k1,59:11644890,26675429:136915
x1,59:11827073,26675429
x1,59:12154753,26675429
x1,59:12456224,26675429
x1,59:13280663,26675429
x1,59:13561815,26675429
k1,59:13698729,26675429:136914
x1,59:14026409,26675429
x1,59:15336457,26675429
k1,59:15473371,26675429:136914
x1,59:16019283,26675429
k1,59:16156198,26675429:136915
x1,59:17284717,26675429
x1,59:17794580,26675429
x1,59:18923099,26675429
k1,59:19060013,26675429:136914
x1,59:19969645,26675429
x1,59:20187877,26675429
k1,60:20187877,26675429:0
)
(1,60:4262629,27461861:15925248,446948,141880
x1,60:5026764,27461861
x1,60:5499923,27461861
x1,60:6774577,27461861
k1,59:6925583,27461861:151006
x1,59:7544239,27461861
x1,59:9109222,27461861
k1,59:9260229,27461861:151007
x1,59:9770092,27461861
x1,59:10061068,27461861
x1,59:11662747,27461861
k1,59:11813753,27461861:151006
x1,59:12796775,27461861
k1,59:12947781,27461861:151006
x1,59:14258483,27461861
k1,59:14409490,27461861:151007
x1,59:14700466,27461861
k1,59:14851472,27461861:151006
x1,59:15542863,27461861
x1,59:15833839,27461861
x1,59:16198205,27461861
x1,59:16509501,27461861
x1,59:17300516,27461861
k1,59:17451523,27461861:151007
x1,59:18871656,27461861
k1,59:19022662,27461861:151006
x1,59:19387038,27461861
x1,59:20187877,27461861
k1,59:20187877,27461861:0
)
(1,60:4262629,28248293:15925248,446948,7531
x1,60:4771837,28248293
x1,60:5882651,28248293
k1,60:20187877,28248293:14305226
g1,60:20187877,28248293
)
(1,62:4262629,29034725:15925248,446948,141880
h1,61:4262629,29034725:983040,0,0
x1,61:6410884,29034725
k1,61:6701665,29034725:290781
x1,61:7138776,29034725
k1,61:7429558,29034725:290782
x1,61:8558068,29034725
k1,61:8848849,29034725:290781
x1,61:9213215,29034725
x1,61:9978006,29034725
x1,61:11470236,29034725
k1,61:11761018,29034725:290782
x1,61:12453064,29034725
k1,61:12743845,29034725:290781
x1,61:13544684,29034725
k1,61:13835466,29034725:290782
x1,61:14053698,29034725
x1,61:14338121,29034725
x1,61:15758272,29034725
k1,61:16049053,29034725:290781
x1,61:16340029,29034725
x1,61:16657885,29034725
x1,61:17458724,29034725
x1,61:18259563,29034725
k1,61:18550345,29034725:290782
x1,61:19096257,29034725
k1,61:19387038,29034725:290781
x1,61:20187877,29034725
k1,61:20187877,29034725:0
)
(1,62:4262629,29821157:15925248,446948,141880
x1,62:5317740,29821157
x1,62:6045835,29821157
k1,61:6232451,29821157:186616
x1,61:7979626,29821157
x1,61:9072097,29821157
k1,61:9258713,29821157:186616
x1,61:10387232,29821157
x1,61:11661230,29821157
k1,61:11847846,29821157:186616
x1,61:12685389,29821157
x1,61:14178274,29821157
k1,61:14426985,29821157:248711
x1,61:15446065,29821157
k1,61:15632681,29821157:186616
x1,61:16688448,29821157
x1,61:16870631,29821157
x1,61:17671470,29821157
k1,61:17858086,29821157:186616
x1,61:19022654,29821157
x1,61:20187877,29821157
k1,61:20187877,29821157:0
)
(1,62:4262629,30607589:15925248,446948,141880
x1,62:5026764,30607589
x1,62:5645420,30607589
x1,62:6118579,30607589
x1,62:7138305,30607589
k1,61:7364994,30607589:226689
x1,61:7946946,30607589
x1,61:9184249,30607589
k1,61:9410937,30607589:226688
x1,61:10248480,30607589
k1,61:10475169,30607589:226689
x1,61:11130529,30607589
k1,61:11357217,30607589:226688
x1,61:14160168,30607589
k1,61:14386857,30607589:226689
x1,61:15078903,30607589
k1,61:15305591,30607589:226688
x1,61:16616311,30607589
k1,61:16843000,30607589:226689
x1,61:17025183,30607589
x1,61:17352863,30607589
x1,61:17654334,30607589
x1,61:18478773,30607589
x1,61:19014853,30607589
k1,61:19241541,30607589:226688
x1,61:20187877,30607589
k1,61:20187877,30607589:0
)
(1,62:4262629,31394021:15925248,446948,141880
x1,62:4917981,31394021
x1,62:5563517,31394021
x1,62:6692036,31394021
k1,61:6998367,31394021:306331
x1,61:7508230,31394021
x1,61:7799206,31394021
x1,61:9145957,31394021
k1,61:9452288,31394021:306331
x1,61:10380272,31394021
k1,61:10722225,31394021:341953
x1,61:12323912,31394021
k1,61:12630243,31394021:306331
x1,61:13103411,31394021
x1,61:13642762,31394021
k1,61:13949093,31394021:306331
x1,61:14240069,31394021
x1,61:14557925,31394021
x1,61:16305100,31394021
k1,61:16611431,31394021:306331
x1,61:17121294,31394021
k1,61:17427625,31394021:306331
x1,61:18228464,31394021
k1,61:18534795,31394021:306331
x1,61:18862475,31394021
k1,61:19168806,31394021:306331
x1,61:19678669,31394021
x1,61:19969645,31394021
x1,61:20187877,31394021
k1,62:20187877,31394021:0
)
(1,62:4262629,32180453:15925248,446948,141880
x1,62:5609380,32180453
k1,61:5805197,32180453:195817
x1,61:6460548,32180453
x1,61:6999907,32180453
x1,61:8165130,32180453
k1,61:8360948,32180453:195818
x1,61:9125083,32180453
x1,61:9743739,32180453
x1,61:10216898,32180453
x1,61:11236624,32180453
k1,61:11432441,32180453:195817
x1,61:12379415,32180453
k1,61:12575233,32180453:195818
x1,61:12902913,32180453
k1,61:13098730,32180453:195817
x1,61:14481522,32180453
k1,61:14677339,32180453:195817
x1,61:15841889,32180453
k1,61:16037707,32180453:195818
x1,61:16747459,32180453
k1,61:16853978,32180453:106519
x1,61:17563730,32180453
k1,61:17862823,32180453:299093
x1,61:18263238,32180453
k1,61:18459055,32180453:195817
x1,61:18932223,32180453
x1,61:20017486,32180453
x1,61:20187877,32180453
k1,61:20187877,32180453:0
)
(1,62:4262629,32966885:15925248,446948,141880
x1,62:5391148,32966885
k1,61:5599424,32966885:208276
x1,61:6254784,32966885
x1,61:6801333,32966885
k1,61:7009609,32966885:208276
x1,61:8320329,32966885
k1,61:8528605,32966885:208276
x1,61:9511627,32966885
k1,61:9719903,32966885:208276
x1,61:10520742,32966885
k1,61:10729018,32966885:208276
x1,61:11384378,32966885
k1,61:11592654,32966885:208276
x1,61:13120933,32966885
x1,61:14286156,32966885
k1,61:14494432,32966885:208276
x1,61:15004295,32966885
x1,61:15295271,32966885
x1,61:16896950,32966885
k1,61:17105226,32966885:208276
x1,61:18378578,32966885
k1,61:18586854,32966885:208276
x1,61:19350989,32966885
x1,61:19969645,32966885
x1,61:20187877,32966885
k1,62:20187877,32966885:0
)
(1,62:4262629,33753317:15925248,446948,141880
x1,62:5536627,33753317
k1,61:5768965,33753317:232338
x1,61:6696949,33753317
k1,61:6946410,33753317:249461
x1,61:8402600,33753317
k1,61:8634937,33753317:232337
x1,61:9435776,33753317
k1,61:9668114,33753317:232338
x1,61:10759938,33753317
x1,61:10965066,33753317
x1,61:12130289,33753317
k1,61:12362626,33753317:232337
x1,61:12981282,33753317
x1,61:13454441,33753317
x1,61:14364719,33753317
x1,61:14983375,33753317
x1,61:16003101,33753317
k1,61:16235439,33753317:232338
x1,61:16708607,33753317
x1,61:17247958,33753317
k1,61:17480295,33753317:232337
x1,61:17771271,33753317
k1,61:18003609,33753317:232338
x1,61:18804448,33753317
x1,61:19532535,33753317
x1,61:20187877,33753317
k1,61:20187877,33753317:0
)
(1,62:4262629,34539749:15925248,446948,141880
x1,62:5391148,34539749
x1,62:6046508,34539749
x1,62:6519667,34539749
x1,62:7539393,34539749
k1,61:7814580,34539749:275187
x1,61:8360492,34539749
k1,61:8635680,34539749:275188
x1,61:9618720,34539749
k1,61:9893907,34539749:275187
x1,61:10403770,34539749
x1,61:10694746,34539749
x1,61:12296425,34539749
k1,61:12571612,34539749:275187
x1,61:13554652,34539749
x1,61:15120282,34539749
k1,61:15395469,34539749:275187
x1,61:16050829,34539749
k1,61:16326017,34539749:275188
x1,61:17708809,34539749
k1,61:17983996,34539749:275187
x1,61:19148546,34539749
k1,61:19423733,34539749:275187
x1,61:20187877,34539749
k1,61:20187877,34539749:0
)
(1,62:4262629,35326181:15925248,446948,141880
x1,62:5864308,35326181
k1,61:6068305,35326181:203997
x1,61:7852185,35326181
k1,61:8056182,35326181:203997
x1,61:8674838,35326181
x1,61:8989414,35326181
x1,61:9270566,35326181
k1,61:9474563,35326181:203997
x1,61:10566378,35326181
x1,61:11767642,35326181
k1,61:11971639,35326181:203997
x1,61:12772478,35326181
k1,61:12976475,35326181:203997
x1,61:13340851,35326181
x1,61:13652147,35326181
x1,61:13933299,35326181
k1,61:14137296,35326181:203997
x1,61:15302519,35326181
k1,61:15506516,35326181:203997
x1,61:16016379,35326181
x1,61:16307355,35326181
x1,61:17909034,35326181
k1,61:18113031,35326181:203997
x1,61:18768391,35326181
x1,61:19569230,35326181
x1,61:19969645,35326181
x1,61:20187877,35326181
k1,62:20187877,35326181:0
)
(1,62:4262629,36112613:15925248,446948,141880
x1,62:5536627,36112613
k1,61:5691201,36112613:154574
x1,61:6400953,36112613
k1,61:6470708,36112613:69755
x1,61:7398692,36112613
k1,61:7598764,36112613:200072
x1,61:8071932,36112613
x1,61:8479554,36112613
k1,61:8634128,36112613:154574
x1,61:9180032,36112613
k1,61:9334606,36112613:154574
x1,61:9771717,36112613
k1,61:9926291,36112613:154574
x1,61:11018762,36112613
x1,61:13093600,36112613
k1,61:13248174,36112613:154574
x1,61:13940220,36112613
k1,61:14094794,36112613:154574
x1,61:14495218,36112613
x1,61:14733769,36112613
x1,61:15534608,36112613
k1,61:15689183,36112613:154575
x1,61:15907415,36112613
h1,61:15907415,36112613:0,0,0
x1,61:16071255,36112613
k1,61:16227682,36112613:156427
x1,61:17028521,36112613
k1,61:17183095,36112613:154574
x1,61:17801751,36112613
x1,61:18092727,36112613
x1,61:18658951,36112613
x1,61:20187877,36112613
k1,61:20187877,36112613:0
)
(1,62:4262629,36899045:15925248,455554,225995
x1,62:5282355,36899045
x1,62:5646721,36899045
x1,62:6484264,36899045
x1,62:7321807,36899045
k1,61:7480938,36899045:159131
x1,61:8281777,36899045
k1,61:8440909,36899045:159132
x1,61:9241748,36899045
x1,61:9569428,36899045
x1,61:10260819,36899045
k1,61:10419950,36899045:159131
x1,61:10710926,36899045
x1,61:11028782,36899045
x1,61:11975118,36899045
x1,61:13067589,36899045
k1,61:13226720,36899045:159131
x1,61:13845376,36899045
x1,61:14864447,36899045
x1,61:15155423,36899045
x1,61:15846814,36899045
k1,61:16005945,36899045:159131
x1,61:16224177,36899045
$1,61:16224177,36899045
(1,61:16224177,36899045:497992,455554,225995
(1,61:16224177,36899045:497992,455554,225995
h1,61:16224177,36899045:78643,0,0
[1,61:16302820,36899045:340706,455554,225995
(1,61:16302820,36641009:340706,197518,0
x1,61:16643526,36641009
)
(1,61:16302820,37125039:340706,197518,0
k1,61:16311710,37125039:8890
x1,61:16618177,37125039
k1,61:16643526,37125039:8889
)
]
h1,61:16643526,36899045:78643,0,0
)
)
$1,61:16722169,36899045
x1,61:16886009,36899045
k1,61:17046082,36899045:160073
x1,61:18647114,36899045
k1,61:18806246,36899045:159132
$1,61:18806246,36899045
x1,61:19225481,36899045
$1,61:19227907,36899045
k1,61:19387038,36899045:159131
x1,61:20187877,36899045
k1,61:20187877,36899045:0
)
(1,62:4262629,37685477:15925248,446948,92400
x1,62:5245661,37685477
k1,61:5503823,37685477:258162
x1,61:6777822,37685477
x1,61:7796893,37685477
k1,61:8055055,37685477:258162
x1,61:9001391,37685477
x1,61:10403181,37685477
k1,61:10684923,37685477:281742
x1,61:11122034,37685477
k1,61:11380195,37685477:258161
x1,61:11998851,37685477
x1,61:13309563,37685477
k1,61:13567725,37685477:258162
x1,61:14259771,37685477
k1,61:14517933,37685477:258162
x1,61:15974115,37685477
k1,61:16232277,37685477:258162
x1,61:16778189,37685477
k1,61:17036351,37685477:258162
x1,61:17837190,37685477
k1,61:18095352,37685477:258162
x1,61:19150463,37685477
x1,61:20187877,37685477
k1,61:20187877,37685477:0
)
(1,62:4262629,38471909:15925248,666981,225995
x1,62:5390493,38471909
x1,61:5997357,38471909
k1,61:6142093,38471909:144736
$1,61:6142093,38471909
x1,61:6447246,38471909
$1,61:6447246,38471909
k1,61:6591983,38471909:144737
x1,61:7137887,38471909
k1,61:7282623,38471909:144736
$1,61:7282623,38471909
x1,61:7701858,38471909
k1,61:7886324,38471909:182040
x1,61:8396050,38471909
k1,61:8578090,38471909:182040
(1,61:8578090,38471909:741448,666981,225995
(1,61:8578090,38471909:741448,666981,225995
h1,61:8578090,38471909:78643,0,0
[1,61:8656733,38471909:584162,666981,225995
(1,61:8656733,38213873:584162,408945,0
k1,61:8696601,38213873:39868
x1,61:8945252,38213873
(1,61:8945252,38016099:255776,211171,0
x1,61:9168260,38016099
)
k1,61:9240895,38213873:39867
)
(1,61:8656733,38697903:584162,295640,0
x1,61:9224435,38697903
)
]
h1,61:9240895,38471909:78643,0,0
)
)
$1,61:9319538,38471909
x1,61:9537770,38471909
k1,61:9682507,38471909:144737
x1,61:10628843,38471909
k1,61:10773579,38471909:144736
x1,61:11428939,38471909
k1,61:11573676,38471909:144737
x1,61:12192332,38471909
x1,61:13029875,38471909
k1,61:13174611,38471909:144736
x1,61:14521354,38471909
k1,61:14666091,38471909:144737
x1,61:15175954,38471909
k1,61:15320690,38471909:144736
x1,61:16740823,38471909
k1,61:16885560,38471909:144737
x1,61:18122863,38471909
x1,61:19105885,38471909
x1,61:20187877,38471909
k1,61:20187877,38471909:0
)
(1,62:4262629,39258341:15925248,446948,141880
x1,62:5973756,39258341
k1,61:6205783,39258341:232027
x1,61:6715646,39258341
k1,61:6947673,39258341:232027
x1,61:8112233,39258341
x1,61:8876368,39258341
x1,61:9204048,39258341
x1,61:9895439,39258341
k1,61:10127467,39258341:232028
x1,61:11037099,39258341
x1,61:11801234,39258341
x1,61:12274393,39258341
x1,61:13549047,39258341
k1,61:13781074,39258341:232027
x1,61:14399730,39258341
x1,61:15964713,39258341
k1,61:16196740,39258341:232027
x1,61:16706603,39258341
x1,61:17417659,39258341
x1,61:18436730,39258341
k1,61:18668757,39258341:232027
x1,61:19324109,39258341
x1,61:19969645,39258341
x1,61:20187877,39258341
k1,62:20187877,39258341:0
)
(1,62:4262629,40044773:15925248,446948,141880
x1,62:5391148,40044773
g1,61:5554988,40044773
x1,61:6064851,40044773
x1,61:6355827,40044773
x1,61:8121346,40044773
k1,62:20187877,40044773:12066531
g1,62:20187877,40044773
)
(1,79:4262629,41093349:15925248,0,0
k1,79:12225253,41093349:7962624
(1,63:12225253,41093349:0,0,0
g1,63:12225253,41093349
g1,63:12225253,41093349
g1,63:11897573,41093349
h1,63:11897573,41093349:0,0,0
g1,63:12225253,41093349
)
k1,79:12225253,41093349:0
g1,79:12225253,41093349
k1,79:20187877,41093349:7962624
)
]
k1,87:20777701,41093349:589824
r1,90:20777701,41093349:0,25242166,141880
k1,87:21367525,41093349:589824
[1,87:21367525,41093349:15925248,25100286,9168
(1,82:21367525,16648423:15925248,446948,141880
h1,81:21367525,16648423:983040,0,0
x1,81:23878853,16648423
k1,81:24022155,16648423:143302
x1,81:24822339,16648423
k1,81:24965641,16648423:143302
x1,81:26021408,16648423
k1,81:26164710,16648423:143302
x1,81:26856756,16648423
x1,81:27512116,16648423
x1,81:28713370,16648423
k1,81:28856672,16648423:143302
x1,81:29766304,16648423
x1,81:30530439,16648423
x1,81:31003598,16648423
x1,81:32278252,16648423
k1,81:32421554,16648423:143302
x1,81:32967466,16648423
k1,81:33110768,16648423:143302
x1,81:34021056,16648423
x1,81:34421471,16648423
x1,81:35331759,16648423
k1,81:35475060,16648423:143301
x1,81:36421396,16648423
k1,81:36564678,16648423:143282
x1,81:36892358,16648423
x1,81:37292773,16648423
k1,82:37292773,16648423:0
)
(1,82:21367525,17434855:15925248,446948,141880
x1,82:21695205,17434855
x1,82:21976357,17434855
x1,82:22194589,17434855
x1,82:23966013,17434855
k1,81:24206267,17434855:240254
x1,81:24824923,17434855
x1,81:26389906,17434855
k1,81:26630159,17434855:240253
x1,81:27140022,17434855
x1,81:27430998,17434855
x1,81:29032677,17434855
k1,81:29272931,17434855:240254
x1,81:29782794,17434855
x1,81:30474850,17434855
x1,81:32003138,17434855
k1,81:32243391,17434855:240253
x1,81:32898751,17434855
k1,81:33139005,17434855:240254
x1,81:33939844,17434855
k1,81:34180097,17434855:240253
x1,81:34507777,17434855
x1,81:35741816,17434855
k1,81:35982070,17434855:240254
x1,81:37074541,17434855
x1,81:37292773,17434855
k1,82:37292773,17434855:0
)
(1,82:21367525,18221287:15925248,446948,141880
x1,82:22168364,18221287
x1,82:22896459,18221287
k1,81:23098617,18221287:202158
x1,81:23644529,18221287
k1,81:23846686,18221287:202157
x1,81:25357286,18221287
k1,81:25559444,18221287:202158
x1,81:27161131,18221287
k1,81:27363288,18221287:202157
x1,81:28309624,18221287
k1,81:28511782,18221287:202158
x1,81:30041371,18221287
k1,81:30243528,18221287:202157
x1,81:31043712,18221287
x1,81:31954000,18221287
x1,81:33082519,18221287
k1,81:33284677,18221287:202158
x1,81:34340444,18221287
k1,81:34542601,18221287:202157
x1,81:35488937,18221287
x1,81:36580752,18221287
k1,81:36782910,18221287:202158
x1,81:37292773,18221287
k1,81:37292773,18221287:0
)
(1,82:21367525,19007719:15925248,446948,9168
x1,82:22168364,19007719
k1,81:22423569,19007719:255205
x1,81:23333857,19007719
x1,81:23989199,19007719
k1,81:24244404,19007719:255205
x1,81:25154036,19007719
x1,81:25918171,19007719
x1,81:26391330,19007719
x1,81:27665984,19007719
k1,81:27921189,19007719:255205
x1,81:28904211,19007719
k1,81:29159416,19007719:255205
x1,81:29923551,19007719
x1,81:30238127,19007719
x1,81:30519279,19007719
k1,81:30774484,19007719:255205
x1,81:31393140,19007719
x1,81:32558363,19007719
k1,81:32813568,19007719:255205
x1,81:34014832,19007719
k1,81:34270037,19007719:255205
x1,81:35690170,19007719
k1,81:35945375,19007719:255205
x1,81:36309751,19007719
x1,81:37292773,19007719
k1,81:37292773,19007719:0
)
(1,82:21367525,19794151:15925248,446948,141880
x1,82:22641524,19794151
k1,81:22925344,19794151:283820
x1,81:24053863,19794151
x1,81:25692245,19794151
k1,81:25976066,19794151:283821
x1,81:26922402,19794151
x1,81:27240258,19794151
x1,81:27685250,19794151
k1,81:28248351,19794151:563101
x1,81:28794263,19794151
x1,81:30195415,19794151
k1,81:30509229,19794151:313814
x1,81:31456203,19794151
k1,81:31740023,19794151:283820
x1,81:32941287,19794151
k1,81:33255102,19794151:313815
x1,81:34092645,19794151
x1,81:34274828,19794151
x1,81:34457011,19794151
x1,81:34768307,19794151
x1,81:35843738,19794151
k1,81:36127558,19794151:283820
x1,81:37074541,19794151
x1,81:37292773,19794151
k1,82:37292773,19794151:0
)
(1,82:21367525,20580583:15925248,450225,141880
x1,82:22496044,20580583
x1,82:22996083,20580583
(1,81:23032455,20577306:218232,446948,0
x1,81:23250687,20577306
)
x1,81:23287059,20580583
k1,81:23489023,20580583:201964
x1,81:23998886,20580583
k1,81:24200850,20580583:201964
x1,81:25074442,20580583
x1,81:26275706,20580583
k1,81:26477670,20580583:201964
x1,81:28006622,20580583
x1,81:28844165,20580583
k1,81:29046128,20580583:201963
x1,81:29555991,20580583
x1,81:29846967,20580583
x1,81:31448646,20580583
k1,81:31650610,20580583:201964
x1,81:32670336,20580583
k1,81:32872300,20580583:201964
x1,81:33673140,20580583
x1,81:35238114,20580583
k1,81:35440078,20580583:201964
x1,81:36058734,20580583
x1,81:37292773,20580583
k1,81:37292773,20580583:0
)
(1,82:21367525,21367015:15925248,446948,141880
x1,82:22514380,21367015
x1,81:22759484,21367015
k1,81:22938223,21367015:178739
x1,81:25194615,21367015
k1,81:25370373,21367015:175758
x1,81:26353388,21367015
k1,81:26529147,21367015:175759
x1,81:27075059,21367015
k1,81:27250818,21367015:175759
x1,81:27578498,21367015
x1,81:28812537,21367015
k1,81:28988296,21367015:175759
x1,81:29170479,21367015
x1,81:29498159,21367015
x1,81:29799630,21367015
x1,81:30474637,21367015
x1,81:31275476,21367015
k1,81:31451235,21367015:175759
x1,81:31961098,21367015
x1,81:32252074,21367015
x1,81:33853753,21367015
k1,81:34029512,21367015:175759
x1,81:34829696,21367015
k1,81:35005455,21367015:175759
x1,81:36170678,21367015
k1,81:36346437,21367015:175759
x1,81:37292773,21367015
k1,81:37292773,21367015:0
)
(1,82:21367525,22153447:15925248,446948,141880
x1,82:21731901,22153447
x1,82:23042603,22153447
k1,81:23257121,22153447:214518
x1,81:24203457,22153447
k1,81:24407840,22153447:204383
x1,81:24917703,22153447
x1,81:25228999,22153447
x1,81:25510151,22153447
k1,81:25714534,22153447:204383
x1,81:26660870,22153447
x1,81:27243468,22153447
x1,81:27571148,22153447
x1,81:27885724,22153447
x1,81:29160378,22153447
k1,81:29364761,22153447:204383
x1,81:30347783,22153447
k1,81:30552166,22153447:204383
x1,81:31352350,22153447
k1,81:31556733,22153447:204383
x1,81:32903476,22153447
k1,81:33107859,22153447:204383
x1,81:33617722,22153447
k1,81:33822105,22153447:204383
x1,81:34440761,22153447
x1,81:35278304,22153447
k1,81:35482687,22153447:204383
x1,81:35992550,22153447
x1,81:36174733,22153447
x1,81:36465709,22153447
x1,81:37292773,22153447
k1,81:37292773,22153447:0
)
(1,82:21367525,22939879:15925248,553676,225995
x1,82:22387251,22939879
x1,82:22751617,22939879
x1,82:23807384,22939879
k1,81:24019346,22939879:211962
x1,81:24565258,22939879
k1,81:24777220,22939879:211962
$1,81:24777220,22939879
x1,81:25286946,22939879
(1,81:25286946,22939879:418521,553676,225995
(1,81:25286946,22939879:418521,553676,225995
h1,81:25286946,22939879:78643,0,0
[1,81:25365589,22939879:261235,553676,225995
(1,81:25365589,22681843:261235,295640,0
x1,81:25626824,22681843
)
(1,81:25365589,23165873:261235,295640,0
x1,81:25626824,23165873
)
]
h1,81:25626824,22939879:78643,0,0
)
)
$1,81:25705467,22939879
k1,81:25917428,22939879:211961
x1,81:26937154,22939879
x1,81:27301520,22939879
x1,81:28612222,22939879
k1,81:28824184,22939879:211962
x1,81:29479544,22939879
k1,81:29691506,22939879:211962
x1,81:30492345,22939879
k1,81:30704307,22939879:211962
x1,81:31322963,22939879
x1,81:32196555,22939879
x1,81:32924650,22939879
x1,81:33688785,22939879
k1,81:33900746,22939879:211961
x1,81:34556106,22939879
x1,81:35522098,22939879
k1,81:35734060,22939879:211962
x1,81:36279972,22939879
k1,81:36491934,22939879:211962
x1,81:37292773,22939879
k1,81:37292773,22939879:0
)
(1,82:21367525,23726311:15925248,550688,141880
x1,82:21986181,23726311
x1,82:22714276,23726311
x1,82:23260188,23726311
x1,82:23574764,23726311
x1,82:23865740,23726311
x1,82:24230106,23726311
x1,82:24541402,23726311
x1,82:24822554,23726311
k1,81:25017796,23726311:195242
x1,81:25308772,23726311
x1,81:25626628,23726311
x1,81:26572964,23726311
x1,81:27665435,23726311
k1,81:27860677,23726311:195242
x1,81:28479333,23726311
x1,81:29498404,23726311
x1,81:29789380,23726311
x1,81:30480771,23726311
k1,81:30676013,23726311:195242
(1,81:30676013,23726311:262144,550688,0
$1,81:30676013,23726311
(1,81:30676013,23488486:262144,312863,0
x1,81:30905389,23488486
)
$1,81:30938157,23726311
)
x1,81:31101997,23726311
k1,81:31399364,23726311:297367
x1,81:32418444,23726311
k1,81:32613686,23726311:195242
x1,81:33050797,23726311
x1,81:34179309,23726311
k1,81:34374551,23726311:195242
x1,81:34920463,23726311
k1,81:35115705,23726311:195242
x1,81:35333937,23726311
x1,81:35909336,23726311
x1,81:36419199,23726311
x1,81:37292773,23726311
k1,81:37292773,23726311:0
)
(1,82:21367525,24512743:15925248,446948,141880
x1,82:22241117,24512743
x1,81:23207764,24512743
k1,81:23401914,24512743:194150
x1,81:24348250,24512743
k1,81:24542400,24512743:194150
x1,81:25452032,24512743
x1,81:26216167,24512743
x1,81:26689326,24512743
x1,81:27709052,24512743
k1,81:27903201,24512743:194149
x1,81:28449113,24512743
k1,81:28643263,24512743:194150
x1,81:28970943,24512743
x1,81:29153126,24512743
x1,81:29464422,24512743
x1,81:29745574,24512743
x1,81:29963806,24512743
x1,81:31735230,24512743
k1,81:31929380,24512743:194150
x1,81:32366491,24512743
k1,81:32560641,24512743:194150
x1,81:33215983,24512743
k1,81:33410132,24512743:194149
x1,81:34210971,24512743
k1,81:34405121,24512743:194150
x1,81:35751872,24512743
k1,81:35946022,24512743:194150
x1,81:37074541,24512743
x1,81:37292773,24512743
k1,82:37292773,24512743:0
)
(1,82:21367525,25299175:15925248,446948,141880
x1,82:22059571,25299175
x1,82:23442362,25299175
k1,81:23570244,25299175:127882
x1,81:24080107,25299175
k1,81:24207990,25299175:127883
x1,81:25008829,25299175
k1,81:25136711,25299175:127882
x1,81:26264567,25299175
k1,81:26392450,25299175:127883
x1,81:26938362,25299175
k1,81:27066244,25299175:127882
x1,81:27903132,25299175
x1,81:28399891,25299175
x1,81:29237434,25299175
k1,81:29365317,25299175:127883
x1,81:30166156,25299175
x1,81:30858202,25299175
x1,81:32405489,25299175
k1,81:32540563,25299175:135074
x1,81:33086467,25299175
k1,81:33214349,25299175:127882
x1,81:33978493,25299175
k1,81:34106376,25299175:127883
x1,81:35344326,25299175
k1,81:35472208,25299175:127882
x1,81:36309751,25299175
x1,81:37292773,25299175
k1,81:37292773,25299175:0
)
(1,82:21367525,26085607:15925248,446948,141880
x1,82:21986181,26085607
x1,82:22496044,26085607
x1,82:22952828,26085607
x1,82:23074076,26085607
k1,81:23317774,26085607:243698
x1,81:24919461,26085607
k1,81:25147188,26085607:227727
x1,81:25584299,26085607
k1,81:25812027,26085607:227728
x1,81:26103003,26085607
k1,81:26330730,26085607:227727
x1,81:27095521,26085607
x1,81:27605384,26085607
x1,81:27969760,26085607
x1,81:29061575,26085607
k1,81:29289302,26085607:227727
x1,81:30126845,26085607
x1,81:30309028,26085607
x1,81:30491211,26085607
x1,81:30802507,26085607
x1,81:31077099,26085607
x1,81:32096825,26085607
k1,81:32324552,26085607:227727
x1,81:33088696,26085607
k1,81:33316423,26085607:227727
x1,81:34117262,26085607
k1,81:34344989,26085607:227727
x1,81:34963645,26085607
x1,81:37292773,26085607
k1,81:37292773,26085607:0
)
(1,82:21367525,26872039:15925248,446948,141880
x1,82:22204413,26872039
x1,82:23878836,26872039
g1,81:24042676,26872039
x1,81:24552539,26872039
g1,81:24716379,26872039
x1,81:25663353,26872039
g1,81:25827193,26872039
x1,81:26773529,26872039
x1,81:27356127,26872039
x1,81:27683807,26872039
x1,81:27998383,26872039
x1,81:29181949,26872039
k1,82:37292773,26872039:8110824
g1,82:37292773,26872039
)
(1,84:21367525,28084454:15925248,446948,141880
h1,83:21367525,28084454:983040,0,0
x1,83:24297629,28084454
k1,83:24535962,28084454:238333
x1,83:25336801,28084454
k1,83:25560236,28084454:223435
x1,83:26506572,28084454
x1,83:26824428,28084454
x1,83:27105580,28084454
k1,83:27329015,28084454:223435
x1,83:28275351,28084454
x1,83:29040142,28084454
x1,83:29331118,28084454
x1,83:29840326,28084454
x1,83:31114980,28084454
k1,83:31338415,28084454:223435
x1,83:32248703,28084454
x1,83:33304470,28084454
k1,83:33527905,28084454:223435
x1,83:34510927,28084454
k1,83:34734362,28084454:223435
x1,83:35098728,28084454
k1,83:35322163,28084454:223435
x1,83:36450682,28084454
k1,83:36674117,28084454:223435
x1,83:37292773,28084454
k1,83:37292773,28084454:0
)
(1,84:21367525,28870886:15925248,446948,141880
x1,84:21986181,28870886
x1,84:22313861,28870886
x1,84:22916133,28870886
x1,84:23389292,28870886
x1,84:24918236,28870886
k1,83:25068744,28870886:150508
x1,83:25578607,28870886
k1,83:25729116,28870886:150509
x1,83:26675452,28870886
x1,83:27949451,28870886
k1,83:28099959,28870886:150508
x1,83:28573118,28870886
x1,83:29046277,28870886
x1,83:29883165,28870886
x1,83:30247531,28870886
x1,83:30558827,28870886
x1,83:30839979,28870886
k1,83:30990488,28870886:150509
x1,83:31754623,28870886
x1,83:32373279,28870886
x1,83:32846438,28870886
x1,83:34339323,28870886
k1,83:34489831,28870886:150508
x1,83:35581646,28870886
x1,83:37292773,28870886
k1,83:37292773,28870886:0
)
(1,84:21367525,29657318:15925248,446948,141880
x1,84:22350547,29657318
k1,83:22587407,29657318:236860
x1,83:22878383,29657318
x1,83:23192959,29657318
x1,83:24017398,29657318
k1,83:24254259,29657318:236861
x1,83:25055098,29657318
k1,83:25291958,29657318:236860
x1,83:25947310,29657318
x1,83:26592846,29657318
x1,83:27721365,29657318
k1,83:27958225,29657318:236860
x1,83:28468088,29657318
x1,83:28759064,29657318
x1,83:30105815,29657318
k1,83:30342676,29657318:236861
x1,83:31143515,29657318
x1,83:32272034,29657318
x1,83:33108922,29657318
x1,83:33230170,29657318
k1,83:33652390,29657318:422220
x1,83:34088854,29657318
k1,83:34325715,29657318:236861
x1,83:35526979,29657318
k1,83:35763839,29657318:236860
x1,83:37074541,29657318
x1,83:37292773,29657318
k1,84:37292773,29657318:0
)
(1,84:21367525,30443750:15925248,446948,141880
x1,84:22277813,30443750
k1,83:22516578,30443750:238765
x1,83:23789930,30443750
k1,83:24028694,30443750:238764
x1,83:24829533,30443750
x1,83:25520924,30443750
k1,83:25759689,30443750:238765
x1,83:26523824,30443750
k1,83:26762588,30443750:238764
x1,83:27272451,30443750
k1,83:27511216,30443750:238765
x1,83:28639735,30443750
x1,83:28821918,30443750
x1,83:29768237,30443750
k1,83:30007001,30443750:238764
x1,83:30807840,30443750
k1,83:31046605,30443750:238765
x1,83:31374285,30443750
x1,83:32608324,30443750
k1,83:32847088,30443750:238764
x1,83:33939559,30443750
x1,83:34740398,30443750
x1,83:35468493,30443750
k1,83:35707258,30443750:238765
x1,83:36253170,30443750
k1,83:36491934,30443750:238764
x1,83:37292773,30443750
k1,83:37292773,30443750:0
)
(1,84:21367525,31230182:15925248,446948,141880
x1,84:22022885,31230182
x1,84:22641541,31230182
x1,84:23369636,31230182
x1,84:24207179,31230182
k1,83:24442292,31230182:235113
x1,83:25243131,31230182
x1,83:26116723,31230182
x1,83:26237971,31230182
k1,83:26490903,31230182:252932
x1,83:27437239,31230182
k1,83:27672352,31230182:235113
x1,83:28800871,31230182
k1,83:29035984,31230182:235113
x1,83:30310000,31230182
k1,83:30545114,31230182:235114
x1,83:31528136,31230182
k1,83:31763249,31230182:235113
x1,83:32564088,31230182
k1,83:32799202,31230182:235114
x1,83:33309065,31230182
x1,83:33782224,31230182
x1,83:34801295,31230182
x1,83:35311158,31230182
x1,83:36075293,31230182
k1,83:36310406,31230182:235113
x1,83:37074541,31230182
x1,83:37292773,31230182
k1,84:37292773,31230182:0
)
(1,84:21367525,32016614:15925248,446948,141880
x1,84:21986181,32016614
x1,84:22459340,32016614
x1,84:23733994,32016614
k1,83:23973930,32016614:239936
x1,83:25430129,32016614
k1,83:25670066,32016614:239937
x1,83:26288722,32016614
k1,83:26528658,32016614:239936
x1,83:28420657,32016614
k1,83:28660593,32016614:239936
x1,83:29606929,32016614
k1,83:29846866,32016614:239937
x1,83:30829888,32016614
k1,83:31069824,32016614:239936
x1,83:31434190,32016614
k1,83:31674127,32016614:239937
x1,83:32802646,32016614
k1,83:33042582,32016614:239936
x1,83:33661238,32016614
k1,83:33901174,32016614:239936
x1,83:34738054,32016614
x1,83:35429445,32016614
k1,83:35669382,32016614:239937
x1,83:36179245,32016614
k1,83:36419181,32016614:239936
x1,83:37074541,32016614
x1,83:37292773,32016614
k1,84:37292773,32016614:0
)
(1,84:21367525,32803046:15925248,446948,141880
x1,84:21986181,32803046
x1,84:23587860,32803046
k1,83:23781720,32803046:193860
x1,83:24582559,32803046
k1,83:24776419,32803046:193860
x1,83:25504514,32803046
x1,83:26596985,32803046
k1,83:26790845,32803046:193860
x1,83:27336757,32803046
k1,83:27530617,32803046:193860
x1,83:28331456,32803046
k1,83:28525315,32803046:193859
x1,83:29872713,32803046
x1,83:31001225,32803046
k1,83:31195085,32803046:193860
x1,83:32141421,32803046
k1,83:32335281,32803046:193860
x1,83:32990641,32803046
x1,83:33791480,32803046
x1,83:34191895,32803046
x1,83:34956030,32803046
k1,83:35149890,32803046:193860
x1,83:35477570,32803046
x1,83:36553001,32803046
k1,83:36746861,32803046:193860
x1,83:37292773,32803046
k1,83:37292773,32803046:0
)
(1,84:21367525,33589478:15925248,446948,141880
x1,84:22168364,33589478
k1,83:22340028,33589478:171664
x1,83:22704404,33589478
x1,83:23505243,33589478
k1,83:23676906,33589478:171663
x1,83:24186114,33589478
x1,83:25296928,33589478
k1,83:25523559,33589478:226631
x1,83:26069471,33589478
k1,83:26241134,33589478:171663
x1,83:27188108,33589478
k1,83:27359772,33589478:171664
x1,83:28488291,33589478
k1,83:28659954,33589478:171663
x1,83:29424098,33589478
k1,83:29595762,33589478:171664
x1,83:31488417,33589478
k1,83:31660080,33589478:171663
x1,83:32315431,33589478
x1,83:32636558,33589478
k1,83:32808222,33589478:171664
x1,83:34009486,33589478
k1,83:34181149,33589478:171663
x1,83:34799805,33589478
x1,83:37292773,33589478
k1,83:37292773,33589478:0
)
(1,84:21367525,34375910:15925248,448587,141880
x1,84:22532748,34375910
k1,83:22707383,34375910:174635
x1,83:23253295,34375910
k1,83:23427930,34375910:174635
x1,83:25029617,34375910
k1,83:25204251,34375910:174634
x1,83:26004435,34375910
k1,83:26179070,34375910:174635
x1,83:27671310,34375910
k1,83:27845945,34375910:174635
x1,83:28501305,34375910
k1,83:28675940,34375910:174635
x1,83:29258548,34375910
x1,83:29689106,34375910
k1,83:29863740,34375910:174634
x1,83:31174460,34375910
x1,83:32412410,34375910
k1,83:32604733,34375910:174635
x1,83:33441621,34375910
x1,83:33950829,34375910
x1,83:34824413,34375910
x1,83:35297572,34375910
x1,83:36572226,34375910
k1,83:36746861,34375910:174635
x1,83:37292773,34375910
k1,83:37292773,34375910:0
)
(1,84:21367525,35162342:15925248,448587,141880
x1,84:22532740,35162342
k1,83:22732906,35162342:200166
x1,83:23533745,35162342
x1,83:24407337,35162342
k1,83:24607503,35162342:200166
x1,83:25153407,35162342
k1,83:25353573,35162342:200166
x1,83:25644549,35162342
k1,83:25844715,35162342:200166
x1,83:26791051,35162342
x1,83:27082027,35162342
x1,83:28065067,35162342
x1,83:28247250,35162342
x1,83:29011385,35162342
k1,83:29211551,35162342:200166
x1,83:29429783,35162342
x1,83:29720759,35162342
x1,83:30505214,35162342
x1,83:31144181,35162342
k1,83:31419993,35162342:275812
x1,83:31710969,35162342
k1,83:31911135,35162342:200166
x1,83:33440717,35162342
k1,83:33640883,35162342:200166
x1,83:34150746,35162342
x1,83:35170465,35162342
x1,83:35764872,35162342
k1,83:35982726,35162342:200166
x1,83:37074541,35162342
x1,83:37292773,35162342
k1,84:37292773,35162342:0
)
(1,84:21367525,35948774:15925248,446948,141880
x1,84:22823724,35948774
k1,83:23067120,35948774:243396
x1,83:23394800,35948774
x1,83:23685776,35948774
x1,83:23997072,35948774
x1,83:24460407,35948774
x1,83:25734423,35948774
k1,83:25977818,35948774:243395
x1,83:26633178,35948774
k1,83:26876574,35948774:243396
x1,83:28150582,35948774
k1,83:28393978,35948774:243396
x1,83:29522506,35948774
x1,83:30359394,35948774
k1,83:30602789,35948774:243395
x1,83:31549125,35948774
k1,83:31792521,35948774:243396
x1,83:32666760,35948774
x1,83:34086255,35948774
k1,83:34329650,35948774:243395
x1,83:35093794,35948774
k1,83:35337190,35948774:243396
x1,83:35628166,35948774
x1,83:35946022,35948774
x1,83:37074541,35948774
x1,83:37292773,35948774
k1,84:37292773,35948774:0
)
(1,84:21367525,36735206:15925248,446948,141880
x1,84:22205068,36735206
k1,83:22361789,36735206:156721
x1,83:23162629,36735206
x1,83:24727603,36735206
k1,83:24884324,36735206:156721
x1,83:26012836,36735206
x1,83:26704227,36735206
k1,83:26860947,36735206:156720
x1,83:27225323,36735206
x1,83:27543179,36735206
x1,83:29072113,36735206
k1,83:29228834,36735206:156721
x1,83:29884194,36735206
x1,83:31485872,36735206
k1,83:31642593,36735206:156721
x1,83:32406737,36735206
k1,83:32563458,36735206:156721
x1,83:33946914,36735206
k1,83:34103627,36735206:156713
x1,83:34758987,36735206
k1,83:34915708,36735206:156721
x1,83:36189716,36735206
k1,83:36346437,36735206:156721
x1,83:37292773,36735206
k1,83:37292773,36735206:0
)
(1,84:21367525,37521638:15925248,446948,141880
x1,84:21840693,37521638
x1,83:22728044,37521638
x1,83:23694036,37521638
k1,83:23844805,37521638:150769
x1,83:24554557,37521638
k1,83:24617970,37521638:63413
x1,83:25491562,37521638
k1,83:25642331,37521638:150769
x1,83:26916338,37521638
k1,83:27067107,37521638:150769
x1,83:27685763,37521638
k1,83:27836532,37521638:150769
x1,83:28346395,37521638
x1,83:28710771,37521638
x1,83:29693793,37521638
k1,83:29844563,37521638:150770
x1,83:30645402,37521638
x1,83:31737873,37521638
k1,83:31888642,37521638:150769
x1,83:33127237,37521638
k1,83:33278006,37521638:150769
x1,83:33823918,37521638
k1,83:33974687,37521638:150769
x1,83:35467573,37521638
k1,83:35618342,37521638:150769
x1,83:36419181,37521638
x1,83:37292773,37521638
k1,83:37292773,37521638:0
)
(1,84:21367525,38308070:15925248,448587,141880
x1,84:21877388,38308070
k1,83:22042351,38308070:164963
x1,83:22843190,38308070
k1,83:23008154,38308070:164964
x1,83:24136010,38308070
k1,83:24300973,38308070:164963
x1,83:24846885,38308070
k1,83:25011848,38308070:164963
x1,83:25848736,38308070
x1,83:26345495,38308070
x1,83:27183038,38308070
k1,83:27348001,38308070:164963
x1,83:28148840,38308070
x1,83:28840886,38308070
x1,83:30406516,38308070
k1,83:30572041,38308070:165525
x1,83:31518377,38308070
k1,83:31683340,38308070:164963
x1,83:32484179,38308070
k1,83:32649143,38308070:164964
x1,83:34178734,38308070
x1,83:35161756,38308070
k1,83:35326719,38308070:164963
x1,83:35836582,38308070
x1,83:37074541,38308070
x1,83:37292773,38308070
k1,84:37292773,38308070:0
)
(1,84:21367525,39094502:15925248,446948,141880
x1,84:22441644,39094502
k1,83:22604967,39094502:163323
x1,83:23114830,39094502
x1,83:23442510,39094502
x1,83:25189030,39094502
k1,83:25352224,39094502:163194
x1,83:26007584,39094502
k1,83:26170778,39094502:163194
x1,83:28427792,39094502
k1,83:28590986,39094502:163194
x1,83:29682810,39094502
k1,83:29846003,39094502:163193
x1,83:30574098,39094502
x1,83:31083961,39094502
x1,83:31540745,39094502
x1,83:32378288,39094502
k1,83:32541482,39094502:163194
x1,83:33233528,39094502
x1,83:34071053,39094502
k1,83:34234247,39094502:163194
x1,83:35144535,39094502
x1,83:36018119,39094502
x1,83:37292773,39094502
k1,83:37292773,39094502:0
)
(1,84:21367525,39880934:15925248,446948,141880
x1,84:22022885,39880934
g1,83:22186725,39880934
x1,83:22842077,39880934
x1,83:23487613,39880934
x1,83:24616132,39880934
g1,83:24779972,39880934
x1,83:25817404,39880934
g1,83:25902604,39880934
x1,83:26940036,39880934
k1,84:37292773,39880934:10352737
g1,84:37292773,39880934
)
(1,87:21367525,41093349:15925248,446948,9168
h1,86:21367525,41093349:983040,0,0
x1,86:23369645,41093349
g1,86:23533485,41093349
x1,86:24371028,41093349
x1,86:25354050,41093349
g1,86:25517890,41093349
x1,86:26063802,41093349
g1,86:26227642,41093349
x1,86:27174616,41093349
g1,86:27338456,41093349
x1,86:28284792,41093349
x1,86:28867390,41093349
x1,86:29195070,41093349
x1,86:29509646,41093349
x1,86:30529372,41093349
g1,86:30693212,41093349
x1,86:31130323,41093349
g1,86:31294163,41093349
x1,86:31840067,41093349
g1,86:32003907,41093349
x1,86:32732002,41093349
x1,86:33241865,41093349
x1,86:34135760,41093349
k1,87:37292773,41093349:3157013
g1,87:37292773,41093349
)
]
(1,87:37292773,41093349:0,298188,141880
h1,87:37292773,41093349:327680,298188,141880
k1,87:37292773,41093349:-327680
)
)
(1,88:4262629,43518181:33030144,65536,0
k1,88:11454302,43518181:7191673
r1,90:30101100,43518181:18646798,32768,-32768
k1,88:37292773,43518181:7191673
)
(1,81:4262629,47981199:33030144,1698382,186779
h1,81:4262629,47981199:524288,0,0
g1,81:4131557,47981199
[1,81:4131557,47981199:33030144,1698382,186779
(1,81:4131557,47981199:33030144,1698382,186779
[1,81:4131557,47981199:33030144,1698382,186779
(1,81:4131557,47981199:33030144,1698382,186779
h1,81:4131557,47981199:524288,0,0
g1,81:4000485,47981199
[1,81:4000485,47981199:15728640,1698382,186779
(1,81:4000485,47981199:15728640,1698382,186779
[1,81:4000485,47981199:15728640,1698382,186779
[1,81:4000485,47981199:15728640,1698382,186779
(1,81:4000485,46736015:15728640,453198,186779
r1,90:4000485,46736015:0,622591,186779
(1,81:4000485,46736015:943720,453198,0
k1,81:4714829,46736015:714344
(1,81:4714829,46736015:229376,453198,0
$1,81:4714829,46736015
(1,81:4714829,46550985:229376,268168,0
x1,81:4911437,46550985
)
$1,81:4944205,46736015
)
)
k1,81:5052263,46736015:108058
(1,81:5052263,46736015:0,435814,0
r1,90:5052263,46736015:0,435814,0
)
x1,81:5984436,46736015
k1,81:6092494,46736015:108058
x1,81:6791362,46736015
k1,81:6899420,46736015:108058
x1,81:8151402,46736015
k1,81:8259460,46736015:108058
x1,81:8900132,46736015
k1,81:9008190,46736015:108058
x1,81:9969202,46736015
x1,81:10784984,46736015
k1,81:10893042,46736015:108058
x1,81:11329772,46736015
k1,81:11437831,46736015:108059
x1,81:13126548,46736015
k1,81:13234606,46736015:108058
x1,81:13875278,46736015
k1,81:13983336,46736015:108058
x1,81:14507624,46736015
x1,81:15148296,46736015
x1,81:15468629,46736015
x1,81:16079938,46736015
k1,81:16187996,46736015:108058
x1,81:16886870,46736015
x1,81:17660188,46736015
k1,81:17768246,46736015:108058
x1,81:18204976,46736015
k1,81:18313034,46736015:108058
x1,81:18807959,46736015
x1,81:19390436,46736015
x1,81:19565022,46736015
x1,81:19729125,46736015
k1,81:19729125,46736015:0
)
(1,81:4000485,47358607:15728640,357558,113504
x1,81:4495410,47358607
x1,81:4786904,47358607
x1,81:5035941,47358607
x1,81:5260863,47358607
k1,81:5400290,47358607:139427
x1,81:5895215,47358607
x1,81:6127996,47358607
x1,81:6580975,47358607
x1,81:7804118,47358607
k1,81:7943545,47358607:139427
x1,81:8351436,47358607
k1,81:8490863,47358607:139427
x1,81:9568270,47358607
k1,81:9707689,47358607:139419
x1,81:10610505,47358607
k1,81:10749932,47358607:139427
x1,81:11244857,47358607
k1,81:11384284,47358607:139427
x1,81:11937922,47358607
x1,81:12578070,47358607
k1,81:12717497,47358607:139427
x1,81:13940122,47358607
k1,81:14079549,47358607:139427
x1,81:14982365,47358607
k1,81:15121792,47358607:139427
x1,81:15296378,47358607
x1,81:15756698,47358607
x1,81:16164589,47358607
x1,81:16863450,47358607
k1,81:17002877,47358607:139427
x1,81:18284227,47358607
k1,81:18423654,47358607:139427
x1,81:18802188,47358607
x1,81:19729125,47358607
k1,81:19729125,47358607:0
)
(1,81:4000485,47981199:15728640,435812,186779
x1,81:4554123,47981199
x1,81:5224158,47981199
g1,81:5355230,47981199
x1,81:5588011,47981199
g1,81:5719083,47981199
x1,81:6010584,47981199
x1,81:6797003,47981199
g1,81:6928075,47981199
x1,81:7335442,47981199
x1,81:8209420,47981199
g1,81:8340492,47981199
x1,81:8777222,47981199
g1,81:8908294,47981199
x1,81:9403219,47981199
x1,81:9665363,47981199
x1,81:9906540,47981199
x1,81:10131462,47981199
x1,81:10306048,47981199
x1,81:11519245,47981199
g1,81:11650317,47981199
x1,81:12261633,47981199
g1,81:12392705,47981199
x1,81:13150286,47981199
g1,81:13281358,47981199
x1,81:13718082,47981199
x1,81:14475139,47981199
r1,90:14475139,47981199:0,186779,186779
r1,90:14475139,47981199:0,622591,186779
k1,81:19729125,47981199:5253986
g1,81:19729125,47981199
)
]
]
)
]
k1,81:37161701,47981199:17432576
g1,81:37161701,47981199
)
]
)
]
k1,81:37292773,47981199:131072
g1,81:37292773,47981199
)
]
(1,90:4262629,49947279:33030144,0,0
h1,90:4262629,49947279:33030144,0,0
)
]
]
!56853
}1
!10
{2
[1,163:4736286,49947279:31135659,47579136,104688
(1,163:4736286,2368143:0,0,0
[1,163:0,2368143:0,0,0
(1,163:0,-2368143:0,0,0
g1,163:0,-2368143
)
]
)
[1,163:2841801,49947279:33030144,47579136,104688
[1,163:2841801,3154575:33030144,786432,0
(1,163:2841801,3154575:33030144,451540,7335
(1,163:2841801,3154575:33030144,451540,7335
x1,163:3169481,3154575
k1,163:17005194,3154575:13835713
g1,163:17136266,3154575
x1,163:17340209,3154575
x1,163:18765213,3154575
g1,163:18896285,3154575
x1,163:19187786,3154575
x1,163:19260662,3154575
g1,163:19391734,3154575
x1,163:20090607,3154575
x1,163:20569807,3154575
x1,163:21905160,3154575
g1,163:22036232,3154575
k1,163:35871945,3154575:13835713
)
)
]
[1,163:2841801,47981199:33030144,44040192,0
[1,78:2841801,10948374:33030144,7007367,0
[1,78:2841801,10948374:33030144,7007367,0
(1,76:2841801,7179718:33030144,3238711,2911031
k1,76:6478641,7179718:3636840
h1,66:6478641,7179718:0,0,0
(1,75:6478641,7179718:25756464,3238711,2911031
$1,75:6478641,7179718
[1,75:6478641,7179718:25756464,3238711,2911031
(1,68:6478641,4555222:25756464,588001,235932
g1,68:6478641,4555222
(1,68:6478641,4555222:2533600,588001,235932
r1,163:6478641,4555222:0,786432,235932
g1,68:6465534,4555222
r1,163:6491748,4555222:26214,823933,235932
g1,68:6478641,4555222
g1,68:6871857,4555222
g1,68:6871857,4555222
g1,68:6871858,4555222
x1,68:8619025,4555222
g1,68:8619025,4555222
g1,68:9012241,4555222
g1,68:8999134,4555222
r1,163:9025348,4555222:26214,823933,235932
g1,68:9012241,4555222
)
g1,68:9012241,4555222
(1,68:9012241,4555222:5136679,588001,235932
g1,68:9405457,4555222
k1,68:9960545,4555222:555088
g1,68:9960546,4555222
x1,68:13200616,4555222
k1,68:13755704,4555222:555088
g1,68:14148920,4555222
g1,68:14135813,4555222
r1,163:14162027,4555222:26214,823933,235932
g1,68:14148920,4555222
)
g1,68:14148920,4555222
(1,68:14148920,4555222:6924838,588001,235932
g1,68:14542136,4555222
g1,68:14542136,4555222
g1,68:14542137,4555222
x1,68:16326000,4555222
g1,68:16489840,4555222
x1,68:18419856,4555222
g1,68:18583696,4555222
x1,68:19129608,4555222
g1,68:19293448,4555222
$1,68:19293448,4555222
(1,68:19293448,4555222:1168862,588001,225995
(1,68:19293448,4555222:1168862,588001,225995
h1,68:19293448,4555222:78643,0,0
[1,68:19372091,4555222:1011576,588001,225995
(1,68:19372091,4262861:1011576,295640,89201
x1,68:19669005,4262861
x1,68:20383667,4262861
)
(1,68:19372091,4781216:1011576,295640,0
k1,68:19729422,4781216:357331
x1,68:20026336,4781216
k1,68:20383667,4781216:357331
)
]
h1,68:20383667,4555222:78643,0,0
)
)
$1,68:20462310,4555222
x1,68:20680542,4555222
g1,68:20680542,4555222
g1,68:21073758,4555222
g1,68:21060651,4555222
r1,163:21086865,4555222:26214,823933,235932
g1,68:21073758,4555222
)
g1,68:21073758,4555222
(1,68:21073758,4555222:11161347,588001,235932
g1,68:21466974,4555222
k1,68:24614981,4555222:3148007
g1,68:24614982,4555222
x1,68:28693882,4555222
k1,68:31841889,4555222:3148007
g1,68:32235105,4555222
g1,68:32221998,4555222
r1,163:32248212,4555222:26214,823933,235932
g1,68:32235105,4555222
)
g1,68:32235105,4555222
)
(1,69:6478641,5371044:25756464,553676,235932
g1,69:6478641,5371044
(1,69:6478641,5371044:2533600,553676,235932
r1,163:6478641,5371044:0,786432,235932
g1,69:6465534,5371044
r1,163:6491748,5371044:26214,789608,235932
g1,69:6478641,5371044
g1,69:6871857,5371044
k1,69:6889873,5371044:18016
g1,69:6889874,5371044
x1,69:8601009,5371044
k1,69:8619025,5371044:18016
g1,69:9012241,5371044
g1,69:8999134,5371044
r1,163:9025348,5371044:26214,789608,235932
g1,69:9012241,5371044
)
g1,69:9012241,5371044
(1,69:9012241,5371044:5136679,553676,235932
g1,69:9405457,5371044
k1,69:10188281,5371044:782824
g1,69:10188282,5371044
x1,69:10515962,5371044
g1,69:10679802,5371044
x1,69:12972880,5371044
k1,69:13755704,5371044:782824
g1,69:14148920,5371044
g1,69:14135813,5371044
r1,163:14162027,5371044:26214,789608,235932
g1,69:14148920,5371044
)
g1,69:14148920,5371044
(1,69:14148920,5371044:6924838,553676,235932
g1,69:14542136,5371044
k1,69:17153082,5371044:2610946
g1,69:17153083,5371044
$1,69:17153083,5371044
(1,69:17153083,5371044:418521,553676,225995
(1,69:17153083,5371044:418521,553676,225995
h1,69:17153083,5371044:78643,0,0
[1,69:17231726,5371044:261235,553676,225995
(1,69:17231726,5113008:261235,295640,0
x1,69:17492961,5113008
)
(1,69:17231726,5597038:261235,295640,0
x1,69:17492961,5597038
)
]
h1,69:17492961,5371044:78643,0,0
)
)
(1,69:17571604,5371044:497992,455554,225995
(1,69:17571604,5371044:497992,455554,225995
h1,69:17571604,5371044:78643,0,0
[1,69:17650247,5371044:340706,455554,225995
(1,69:17650247,5113008:340706,197518,0
x1,69:17990953,5113008
)
(1,69:17650247,5597038:340706,197518,0
k1,69:17659137,5597038:8890
x1,69:17965604,5597038
k1,69:17990953,5597038:8889
)
]
h1,69:17990953,5371044:78643,0,0
)
)
$1,69:18069596,5371044
k1,69:20680542,5371044:2610946
g1,69:21073758,5371044
g1,69:21060651,5371044
r1,163:21086865,5371044:26214,789608,235932
g1,69:21073758,5371044
)
g1,69:21073758,5371044
(1,69:21073758,5371044:11161347,553676,235932
g1,69:21466974,5371044
k1,69:23805924,5371044:2338950
g1,69:23805925,5371044
x1,69:25116645,5371044
g1,69:25280485,5371044
x1,69:25608165,5371044
g1,69:25772005,5371044
x1,69:28574956,5371044
g1,69:28738796,5371044
x1,69:29502940,5371044
k1,69:31841889,5371044:2338949
g1,69:32235105,5371044
g1,69:32221998,5371044
r1,163:32248212,5371044:26214,789608,235932
g1,69:32235105,5371044
)
g1,69:32235105,5371044
)
(1,70:6478641,6323871:25756464,690681,235932
g1,70:6478641,6323871
(1,70:6478641,6323871:2533600,690681,235932
r1,163:6478641,6323871:0,786432,235932
g1,70:6465534,6323871
r1,163:6491748,6323871:26214,926613,235932
g1,70:6478641,6323871
g1,70:6871857,6323871
k1,70:6889873,6323871:18016
g1,70:6889874,6323871
x1,70:8601009,6323871
k1,70:8619025,6323871:18016
g1,70:9012241,6323871
g1,70:8999134,6323871
r1,163:9025348,6323871:26214,926613,235932
g1,70:9012241,6323871
)
g1,70:9012241,6323871
(1,70:9012241,6323871:5136679,690681,235932
g1,70:9405457,6323871
k1,70:10060817,6323871:655360
g1,70:10060818,6323871
x1,70:10388498,6323871
g1,70:10552338,6323871
x1,70:13100344,6323871
k1,70:13755704,6323871:655360
g1,70:14148920,6323871
g1,70:14135813,6323871
r1,163:14162027,6323871:26214,926613,235932
g1,70:14148920,6323871
)
g1,70:14148920,6323871
(1,70:14148920,6323871:6924838,690681,235932
g1,70:14542136,6323871
k1,70:15422203,6323871:880067
g1,70:15422204,6323871
$1,70:15422204,6323871
x1,70:17424699,6323871
g1,70:17533923,6323871
(1,70:17533923,6323871:764583,69176,0
x1,70:17715968,6323871
g1,70:17825192,6323871
x1,70:18007237,6323871
g1,70:18116461,6323871
x1,70:18298506,6323871
)
g1,70:18407730,6323871
(1,70:18407730,6323871:300375,557059,229380
$1,70:18407730,6323871
(1,70:18407730,6323871:300375,557059,229380
(1,70:18407730,5793025:300375,26213,760226
x1,70:18708105,5793025
)
v1,70:18708105,6323871:0,557055,229374
h1,70:18708105,6323871:0,0,0
)
$1,70:18708105,6323871
)
(1,70:18708105,6323871:497992,455554,225995
(1,70:18708105,6323871:497992,455554,225995
h1,70:18708105,6323871:78643,0,0
[1,70:18786748,6323871:340706,455554,225995
(1,70:18786748,6065835:340706,197518,0
x1,70:19127454,6065835
)
(1,70:18786748,6549865:340706,197518,0
k1,70:18795638,6549865:8890
x1,70:19102105,6549865
k1,70:19127454,6549865:8889
)
]
h1,70:19127454,6323871:78643,0,0
)
)
(1,70:19206097,6323871:300375,557059,229380
$1,70:19206097,6323871
(1,70:19206097,6323871:300375,557059,229380
(1,70:19206097,5793025:300375,26213,760226
x1,70:19506472,5793025
)
v1,70:19506472,6323871:0,557055,229374
h1,70:19506472,6323871:0,0,0
)
$1,70:19506472,6323871
)
(1,70:19506472,5928830:294003,295640,0
x1,70:19767707,5928830
)
$1,70:19800475,6323871
k1,70:20680542,6323871:880067
g1,70:21073758,6323871
g1,70:21060651,6323871
r1,163:21086865,6323871:26214,926613,235932
g1,70:21073758,6323871
)
g1,70:21073758,6323871
(1,70:21073758,6323871:11161347,690681,235932
g1,70:21466974,6323871
g1,70:21466974,6323871
g1,70:21466975,6323871
x1,70:22777695,6323871
g1,70:22941535,6323871
x1,70:23269215,6323871
g1,70:23433055,6323871
x1,70:26235997,6323871
g1,70:26399837,6323871
x1,70:27163981,6323871
g1,70:27327821,6323871
x1,70:27510004,6323871
g1,70:27673844,6323871
x1,70:30913905,6323871
g1,70:31077745,6323871
x1,70:31841889,6323871
g1,70:31841889,6323871
g1,70:32235105,6323871
g1,70:32221998,6323871
r1,163:32248212,6323871:26214,926613,235932
g1,70:32235105,6323871
)
g1,70:32235105,6323871
)
(1,71:6478641,7276698:25756464,690681,235932
g1,71:6478641,7276698
(1,71:6478641,7276698:2533600,690681,235932
r1,163:6478641,7276698:0,786432,235932
g1,71:6465534,7276698
r1,163:6491748,7276698:26214,926613,235932
g1,71:6478641,7276698
g1,71:6871857,7276698
k1,71:6889873,7276698:18016
g1,71:6889874,7276698
x1,71:8601009,7276698
k1,71:8619025,7276698:18016
g1,71:9012241,7276698
g1,71:8999134,7276698
r1,163:9025348,7276698:26214,926613,235932
g1,71:9012241,7276698
)
g1,71:9012241,7276698
(1,71:9012241,7276698:5136679,690681,235932
g1,71:9405457,7276698
k1,71:9896977,7276698:491520
g1,71:9896978,7276698
x1,71:10552338,7276698
g1,71:10716178,7276698
x1,71:13264184,7276698
k1,71:13755704,7276698:491520
g1,71:14148920,7276698
g1,71:14135813,7276698
r1,163:14162027,7276698:26214,926613,235932
g1,71:14148920,7276698
)
g1,71:14148920,7276698
(1,71:14148920,7276698:6924838,690681,235932
g1,71:14542136,7276698
k1,71:15422203,7276698:880067
g1,71:15422204,7276698
$1,71:15422204,7276698
x1,71:17424699,7276698
g1,71:17533923,7276698
(1,71:17533923,7276698:764583,69176,0
x1,71:17715968,7276698
g1,71:17825192,7276698
x1,71:18007237,7276698
g1,71:18116461,7276698
x1,71:18298506,7276698
)
g1,71:18407730,7276698
(1,71:18407730,7276698:300375,557059,229380
$1,71:18407730,7276698
(1,71:18407730,7276698:300375,557059,229380
(1,71:18407730,6745852:300375,26213,760226
x1,71:18708105,6745852
)
v1,71:18708105,7276698:0,557055,229374
h1,71:18708105,7276698:0,0,0
)
$1,71:18708105,7276698
)
(1,71:18708105,7276698:497992,455554,225995
(1,71:18708105,7276698:497992,455554,225995
h1,71:18708105,7276698:78643,0,0
[1,71:18786748,7276698:340706,455554,225995
(1,71:18786748,7018662:340706,197518,0
x1,71:19127454,7018662
)
(1,71:18786748,7502692:340706,197518,0
k1,71:18795638,7502692:8890
x1,71:19102105,7502692
k1,71:19127454,7502692:8889
)
]
h1,71:19127454,7276698:78643,0,0
)
)
(1,71:19206097,7276698:300375,557059,229380
$1,71:19206097,7276698
(1,71:19206097,7276698:300375,557059,229380
(1,71:19206097,6745852:300375,26213,760226
x1,71:19506472,6745852
)
v1,71:19506472,7276698:0,557055,229374
h1,71:19506472,7276698:0,0,0
)
$1,71:19506472,7276698
)
(1,71:19506472,6881657:294003,295640,0
x1,71:19767707,6881657
)
$1,71:19800475,7276698
k1,71:20680542,7276698:880067
g1,71:21073758,7276698
g1,71:21060651,7276698
r1,163:21086865,7276698:26214,926613,235932
g1,71:21073758,7276698
)
g1,71:21073758,7276698
(1,71:21073758,7276698:11161347,690681,235932
g1,71:21466974,7276698
k1,71:22895641,7276698:1428667
g1,71:22895642,7276698
x1,71:24206362,7276698
g1,71:24370202,7276698
x1,71:24697882,7276698
g1,71:24861722,7276698
x1,71:27063713,7276698
g1,71:27227553,7276698
x1,71:29485238,7276698
g1,71:29649078,7276698
x1,71:30413222,7276698
k1,71:31841889,7276698:1428667
g1,71:32235105,7276698
g1,71:32221998,7276698
r1,163:32248212,7276698:26214,926613,235932
g1,71:32235105,7276698
)
g1,71:32235105,7276698
)
(1,72:6478641,8229525:25756464,690681,235932
g1,72:6478641,8229525
(1,72:6478641,8229525:2533600,690681,235932
r1,163:6478641,8229525:0,786432,235932
g1,72:6465534,8229525
r1,163:6491748,8229525:26214,926613,235932
g1,72:6478641,8229525
g1,72:6871857,8229525
k1,72:6889873,8229525:18016
g1,72:6889874,8229525
x1,72:8601009,8229525
k1,72:8619025,8229525:18016
g1,72:9012241,8229525
g1,72:8999134,8229525
r1,163:9025348,8229525:26214,926613,235932
g1,72:9012241,8229525
)
g1,72:9012241,8229525
(1,72:9012241,8229525:5136679,690681,235932
g1,72:9405457,8229525
k1,72:9733137,8229525:327680
g1,72:9733138,8229525
x1,72:10716178,8229525
g1,72:10880018,8229525
x1,72:13428024,8229525
k1,72:13755704,8229525:327680
g1,72:14148920,8229525
g1,72:14135813,8229525
r1,163:14162027,8229525:26214,926613,235932
g1,72:14148920,8229525
)
g1,72:14148920,8229525
(1,72:14148920,8229525:6924838,690681,235932
g1,72:14542136,8229525
k1,72:15422203,8229525:880067
g1,72:15422204,8229525
$1,72:15422204,8229525
x1,72:17424699,8229525
g1,72:17533923,8229525
(1,72:17533923,8229525:764583,69176,0
x1,72:17715968,8229525
g1,72:17825192,8229525
x1,72:18007237,8229525
g1,72:18116461,8229525
x1,72:18298506,8229525
)
g1,72:18407730,8229525
(1,72:18407730,8229525:300375,557059,229380
$1,72:18407730,8229525
(1,72:18407730,8229525:300375,557059,229380
(1,72:18407730,7698679:300375,26213,760226
x1,72:18708105,7698679
)
v1,72:18708105,8229525:0,557055,229374
h1,72:18708105,8229525:0,0,0
)
$1,72:18708105,8229525
)
(1,72:18708105,8229525:497992,455554,225995
(1,72:18708105,8229525:497992,455554,225995
h1,72:18708105,8229525:78643,0,0
[1,72:18786748,8229525:340706,455554,225995
(1,72:18786748,7971489:340706,197518,0
x1,72:19127454,7971489
)
(1,72:18786748,8455519:340706,197518,0
k1,72:18795638,8455519:8890
x1,72:19102105,8455519
k1,72:19127454,8455519:8889
)
]
h1,72:19127454,8229525:78643,0,0
)
)
(1,72:19206097,8229525:300375,557059,229380
$1,72:19206097,8229525
(1,72:19206097,8229525:300375,557059,229380
(1,72:19206097,7698679:300375,26213,760226
x1,72:19506472,7698679
)
v1,72:19506472,8229525:0,557055,229374
h1,72:19506472,8229525:0,0,0
)
$1,72:19506472,8229525
)
(1,72:19506472,7834484:294003,295640,0
x1,72:19767707,7834484
)
$1,72:19800475,8229525
k1,72:20680542,8229525:880067
g1,72:21073758,8229525
g1,72:21060651,8229525
r1,163:21086865,8229525:26214,926613,235932
g1,72:21073758,8229525
)
g1,72:21073758,8229525
(1,72:21073758,8229525:11161347,690681,235932
g1,72:21466974,8229525
k1,72:24188324,8229525:2721350
g1,72:24188325,8229525
x1,72:25499045,8229525
g1,72:25662885,8229525
x1,72:25990565,8229525
g1,72:26154405,8229525
x1,72:28192556,8229525
g1,72:28356396,8229525
x1,72:29120540,8229525
k1,72:31841889,8229525:2721349
g1,72:32235105,8229525
g1,72:32221998,8229525
r1,163:32248212,8229525:26214,926613,235932
g1,72:32235105,8229525
)
g1,72:32235105,8229525
)
(1,73:6478641,9042171:25756464,550500,235932
g1,73:6478641,9042171
(1,73:6478641,9042171:2533600,550500,235932
r1,163:6478641,9042171:0,786432,235932
g1,73:6465534,9042171
r1,163:6491748,9042171:26214,786432,235932
g1,73:6478641,9042171
g1,73:6871857,9042171
k1,73:6889873,9042171:18016
g1,73:6889874,9042171
x1,73:8601009,9042171
k1,73:8619025,9042171:18016
g1,73:9012241,9042171
g1,73:8999134,9042171
r1,163:9025348,9042171:26214,786432,235932
g1,73:9012241,9042171
)
g1,73:9012241,9042171
(1,73:9012241,9042171:5136679,550500,235932
g1,73:9405457,9042171
g1,73:9405457,9042171
g1,73:9405458,9042171
x1,73:11043858,9042171
g1,73:11207698,9042171
x1,73:13755704,9042171
g1,73:13755704,9042171
g1,73:14148920,9042171
g1,73:14135813,9042171
r1,163:14162027,9042171:26214,786432,235932
g1,73:14148920,9042171
)
g1,73:14148920,9042171
(1,73:14148920,9042171:6924838,550500,235932
g1,73:14542136,9042171
k1,73:17101613,9042171:2559477
g1,73:17101614,9042171
$1,73:17101614,9042171
x1,73:18121066,9042171
$1,73:18121066,9042171
k1,73:20680542,9042171:2559476
g1,73:21073758,9042171
g1,73:21060651,9042171
r1,163:21086865,9042171:26214,786432,235932
g1,73:21073758,9042171
)
g1,73:21073758,9042171
(1,73:21073758,9042171:11161347,550500,235932
g1,73:21466974,9042171
k1,73:26144705,9042171:4677731
g1,73:26144706,9042171
$1,73:26144706,9042171
x1,73:27164158,9042171
$1,73:27164158,9042171
k1,73:31841889,9042171:4677731
g1,73:32235105,9042171
g1,73:32221998,9042171
r1,163:32248212,9042171:26214,786432,235932
g1,73:32235105,9042171
)
g1,73:32235105,9042171
)
(1,75:6478641,9854817:25756464,550500,235932
g1,74:6478641,9854817
(1,74:6478641,9854817:2533600,550500,235932
r1,163:6478641,9854817:0,786432,235932
g1,74:6465534,9854817
r1,163:6491748,9854817:26214,786432,235932
g1,74:6478641,9854817
g1,74:6871857,9854817
k1,74:7308537,9854817:436680
g1,74:7308538,9854817
$1,74:7308538,9854817
(1,74:7308538,9854817:764583,291271,0
x1,74:7490583,9854817
g1,74:7599807,9854817
x1,74:7781852,9854817
g1,74:7891076,9854817
x1,74:8073121,9854817
)
g1,74:8182345,9854817
$1,74:8182345,9854817
k1,74:8619025,9854817:436680
g1,74:9012241,9854817
g1,74:8999134,9854817
r1,163:9025348,9854817:26214,786432,235932
g1,74:9012241,9854817
)
g1,74:9012241,9854817
(1,74:9012241,9854817:5136679,550500,235932
g1,74:9405457,9854817
k1,74:11143677,9854817:1738220
g1,74:11143678,9854817
$1,74:11143678,9854817
(1,74:11143678,9854817:764583,291271,0
x1,74:11325723,9854817
g1,74:11434947,9854817
x1,74:11616992,9854817
g1,74:11726216,9854817
x1,74:11908261,9854817
)
g1,74:12017485,9854817
$1,74:12017485,9854817
k1,74:13755704,9854817:1738219
g1,74:14148920,9854817
g1,74:14135813,9854817
r1,163:14162027,9854817:26214,786432,235932
g1,74:14148920,9854817
)
g1,74:14148920,9854817
(1,74:14148920,9854817:6924838,550500,235932
g1,74:14542136,9854817
k1,74:17174435,9854817:2632299
g1,74:17174436,9854817
$1,74:17174436,9854817
(1,74:17174436,9854817:764583,291271,0
x1,74:17356481,9854817
g1,74:17465705,9854817
x1,74:17647750,9854817
g1,74:17756974,9854817
x1,74:17939019,9854817
)
g1,74:18048243,9854817
$1,74:18048243,9854817
k1,74:20680542,9854817:2632299
g1,74:21073758,9854817
g1,74:21060651,9854817
r1,163:21086865,9854817:26214,786432,235932
g1,74:21073758,9854817
)
g1,74:21073758,9854817
(1,75:21073758,9854817:11161347,550500,235932
g1,74:21466974,9854817
k1,74:26217528,9854817:4750554
g1,74:26217529,9854817
$1,74:26217529,9854817
(1,74:26217529,9854817:764583,291271,0
x1,74:26399574,9854817
g1,74:26508798,9854817
x1,74:26690843,9854817
g1,74:26800067,9854817
x1,74:26982112,9854817
)
g1,74:27091336,9854817
$1,74:27091336,9854817
k1,75:31841889,9854817:4750553
g1,75:32235105,9854817
g1,75:32221998,9854817
r1,163:32248212,9854817:26214,786432,235932
g1,75:32235105,9854817
)
g1,75:32235105,9854817
)
]
$1,75:32235105,7179718
)
k1,76:32235105,7179718:0
g1,76:32235105,7179718
k1,76:35871945,7179718:3636840
)
(1,76:2841801,10820682:33030144,402253,127692
k1,76:10493559,10820682:7651758
h1,76:10493559,10820682:0,0,0
(1,76:10493559,10820682:17726629,402253,127692
x1,76:10883432,10820682
x1,76:12182792,10820682
g1,76:12330248,10820682
x1,76:12733095,10820682
g1,76:12951548,10820682
x1,76:14754031,10820682
x1,76:16184338,10820682
g1,76:16331794,10820682
x1,76:16790671,10820682
g1,76:16938127,10820682
x1,76:17658882,10820682
g1,76:17806338,10820682
x1,76:19706135,10820682
g1,76:19853591,10820682
$1,76:19853591,10820682
x1,76:20142651,10820682
g1,76:20298525,10820682
x1,76:20770017,10820682
g1,76:20904729,10820682
x1,76:21207831,10820682
$1,76:21207831,10820682
g1,76:21355287,10820682
x1,76:21781130,10820682
g1,76:21928586,10820682
x1,76:22223498,10820682
x1,76:23650263,10820682
g1,76:23797719,10820682
x1,76:24846420,10820682
g1,76:24993876,10820682
x1,76:26467831,10820682
g1,76:26615287,10820682
x1,76:28220188,10820682
)
g1,76:28220188,10820682
k1,76:35871945,10820682:7651757
)
]
]
(1,161:2841801,31788822:33030144,19529728,141880
[1,161:2841801,31788822:15925248,19529728,127692
(1,95:3923141,12914454:14843908,402253,127692
(1,94:3923141,12914454:0,380108,6778
g1,94:3923141,12914454
g1,94:3169481,12914454
g1,94:2841801,12914454
(1,94:2841801,12914454:753660,380108,6778
k1,94:3144903,12914454:303102
$1,94:3144903,12914454
x1,94:3448005,12914454
$1,94:3448005,12914454
x1,94:3595461,12914454
)
g1,94:3923141,12914454
)
x1,94:4300032,12914454
k1,94:4608947,12914454:308915
x1,94:7131602,12914454
x1,94:7255470,12914454
k1,94:7604750,12914454:349280
x1,94:8325513,12914454
k1,94:8634428,12914454:308915
x1,94:11026144,12914454
x1,94:14990301,12914454
k1,94:15299216,12914454:308915
x1,94:16150918,12914454
k1,94:16459833,12914454:308915
x1,94:17180588,12914454
k1,94:17489503,12914454:308915
x1,94:18570640,12914454
x1,94:18767049,12914454
k1,95:18767049,12914454:0
)
(1,95:3923141,13635350:14843908,406386,127692
x1,95:5069739,13635350
k1,94:5339021,13635350:269282
x1,94:6158280,13635350
x1,94:7337912,13635350
k1,94:7607195,13635350:269283
x1,94:8098516,13635350
k1,94:8367798,13635350:269282
x1,94:9088553,13635350
k1,94:9357836,13635350:269283
x1,94:10405938,13635350
x1,94:11503592,13635350
k1,94:11803331,13635350:299739
x1,94:12426181,13635350
x1,94:13095038,13635350
k1,94:13364320,13635350:269282
x1,94:14019606,13635350
x1,94:14299772,13635350
x1,94:14408895,13635350
k1,94:14678178,13635350:269283
x1,94:15415458,13635350
k1,94:15715196,13635350:299738
x1,94:17435118,13635350
k1,94:17734857,13635350:299739
x1,94:18767049,13635350
k1,94:18767049,13635350:0
)
(1,95:3923141,14356246:14843908,402253,127692
x1,95:6954791,14356246
x1,94:10106798,14356246
x1,94:11283485,14356246
x1,94:11563651,14356246
x1,94:13442246,14356246
k1,95:18767049,14356246:5324803
g1,95:18767049,14356246
)
(1,101:3923141,15219137:14843908,402253,127692
(1,96:3923141,15219137:0,380108,6778
g1,96:3923141,15219137
g1,96:3169481,15219137
g1,96:2841801,15219137
(1,96:2841801,15219137:753660,380108,6778
k1,96:3144903,15219137:303102
$1,96:3144903,15219137
x1,96:3448005,15219137
$1,96:3448005,15219137
x1,96:3595461,15219137
)
g1,96:3923141,15219137
)
x1,96:4496448,15219137
k1,97:4692942,15219137:196494
x1,97:5282758,15219137
x1,97:5708601,15219137
x1,97:7363045,15219137
k1,97:7571799,15219137:208754
x1,97:7899737,15219137
k1,98:7571799,15219137:-8842
x1,98:9136005,15219137
k1,98:9332499,15219137:196494
x1,98:9627411,15219137
x1,98:10577019,15219137
k1,98:10773513,15219137:196494
x1,98:11789180,15219137
x1,98:12935778,15219137
k1,98:13132272,15219137:196494
x1,98:13886061,15219137
x1,98:15065693,15219137
k1,98:15262188,15219137:196495
x1,98:15753509,15219137
k1,98:15950003,15219137:196494
x1,98:16670758,15219137
k1,98:16867252,15219137:196494
x1,98:17816851,15219137
x1,98:18767049,15219137
k1,98:18767049,15219137:0
)
(1,101:3923141,15940033:14843908,406386,127692
x1,101:5069747,15940033
x1,99:5178870,15940033
k1,99:5334390,15940033:155520
x1,99:5957240,15940033
x1,99:6626097,15940033
k1,99:6781618,15940033:155521
x1,99:7895190,15940033
k1,99:8050710,15940033:155520
x1,99:8640534,15940033
k1,99:8796055,15940033:155521
x1,99:10515977,15940033
k1,99:10673513,15940033:157536
x1,99:11705705,15940033
k1,99:11863242,15940033:157537
x1,99:14894892,15940033
k1,100:11863242,15940033:-10613
x1,100:18767049,15940033
k1,101:18767049,15940033:0
)
(1,101:3923141,16660929:14843908,402253,8251
x1,101:5840069,16660929
k1,101:18767049,16660929:12926980
g1,101:18767049,16660929
)
(1,103:3923141,17523819:14843908,402253,127692
(1,102:3923141,17523819:0,380108,6778
g1,102:3923141,17523819
g1,102:3169481,17523819
g1,102:2841801,17523819
(1,102:2841801,17523819:753660,380108,6778
k1,102:3144903,17523819:303102
$1,102:3144903,17523819
x1,102:3448005,17523819
$1,102:3448005,17523819
x1,102:3595461,17523819
)
g1,102:3923141,17523819
)
x1,102:4464005,17523819
k1,102:4733650,17523819:269645
x1,102:5815377,17523819
x1,102:6536132,17523819
x1,102:6732541,17523819
x1,102:7928690,17523819
k1,102:8228882,17523819:300192
x1,102:9310019,17523819
x1,102:10456617,17523819
k1,102:10726262,17523819:269645
x1,102:12331745,17523819
k1,102:12601391,17523819:269646
x1,102:13420650,17523819
x1,102:14600282,17523819
k1,102:14869927,17523819:269645
x1,102:15361248,17523819
k1,102:15630893,17523819:269645
x1,102:16351648,17523819
k1,102:16621293,17523819:269645
x1,102:17669395,17523819
x1,102:18767049,17523819
k1,102:18767049,17523819:0
)
(1,103:3923141,18244715:14843908,406386,127692
x1,103:4545991,18244715
x1,102:5214848,18244715
g1,102:5362304,18244715
x1,102:6017590,18244715
x1,102:6297756,18244715
x1,102:6406879,18244715
g1,102:6554335,18244715
x1,102:7586527,18244715
g1,102:7733983,18244715
x1,102:9306449,18244715
g1,102:9453905,18244715
x1,102:10486097,18244715
k1,103:18767049,18244715:8280952
g1,103:18767049,18244715
)
(1,110:3923141,19107606:14843908,402253,127692
(1,104:3923141,19107606:0,380108,6778
g1,104:3923141,19107606
g1,104:3169481,19107606
g1,104:2841801,19107606
(1,104:2841801,19107606:753660,380108,6778
k1,104:3144903,19107606:303102
$1,104:3144903,19107606
x1,104:3448005,19107606
$1,104:3448005,19107606
x1,104:3595461,19107606
)
g1,104:3923141,19107606
)
x1,104:4398535,19107606
k1,105:4742634,19107606:344099
x1,105:5364893,19107606
x1,105:6576969,19107606
k1,105:6921068,19107606:344099
x1,105:7772770,19107606
k1,105:8116869,19107606:344099
x1,105:8624706,19107606
k1,105:8968805,19107606:344099
x1,105:11148178,19107606
k1,105:11541438,19107606:393260
x1,105:12458609,19107606
k1,106:12802708,19107606:344099
x1,106:13523471,19107606
x1,106:13785349,19107606
x1,106:14408191,19107606
x1,106:14572156,19107606
x1,106:15259877,19107606
k1,106:15603976,19107606:344099
x1,106:15898888,19107606
x1,106:16866775,19107606
k1,106:17210874,19107606:344099
x1,106:17702195,19107606
k1,106:18046294,19107606:344099
x1,106:18767049,19107606
k1,106:18767049,19107606:0
)
(1,110:3923141,19828502:14843908,402253,127692
x1,110:4872740,19828502
x1,110:5822938,19828502
k1,106:6193076,19828502:370138
x1,106:6880806,19828502
x1,106:7372127,19828502
k1,106:7742265,19828502:370138
x1,106:8168108,19828502
k1,106:8538245,19828502:370137
x1,106:8833157,19828502
x1,106:9782765,19828502
k1,106:10152903,19828502:370138
x1,106:10578746,19828502
x1,106:12315184,19828502
k1,106:12685322,19828502:370138
x1,106:13144199,19828502
k1,106:13514337,19828502:370138
x1,106:14873876,19828502
k1,106:15244013,19828502:370137
x1,106:15866863,19828502
k1,107:15244013,19828502:-2946
x1,107:16535720,19828502
k1,107:16905858,19828502:370138
x1,107:18003503,19828502
k1,107:18373641,19828502:370138
x1,107:18767049,19828502
k1,110:18767049,19828502:0
)
(1,110:3923141,20549398:14843908,406386,127692
x1,110:4807877,20549398
k1,107:4953243,20549398:145366
x1,107:6673165,20549398
k1,107:6818950,20549398:145785
x1,107:7851142,20549398
k1,107:7996926,20549398:145784
x1,107:11028576,20549398
k1,108:7996926,20549398:-10613
x1,108:14933790,20549398
x1,108:18767049,20549398
k1,110:18767049,20549398:0
)
(1,110:3923141,21270294:14843908,402253,127692
x1,110:4348992,21270294
g1,108:4496448,21270294
x1,108:5740960,21270294
k1,109:4496448,21270294:-14746
x1,109:7233202,21270294
x1,109:10051375,21270294
g1,109:10198831,21270294
x1,109:11443351,21270294
x1,109:12573449,21270294
k1,110:18767049,21270294:6193600
g1,110:18767049,21270294
)
(1,118:3923141,22133185:14843908,402253,127692
(1,112:3923141,22133185:0,380108,6778
g1,112:3923141,22133185
g1,112:3169481,22133185
g1,112:2841801,22133185
(1,112:2841801,22133185:753660,380108,6778
k1,112:3144903,22133185:303102
$1,112:3144903,22133185
x1,112:3448005,22133185
$1,112:3448005,22133185
x1,112:3595461,22133185
)
g1,112:3923141,22133185
)
x1,112:4398535,22133185
k1,113:4742943,22133185:344408
x1,113:5365202,22133185
x1,113:6724734,22133185
k1,113:7118379,22133185:393645
x1,113:8494428,22133185
x1,113:10656694,22133185
k1,114:11001101,22133185:344407
x1,114:11688822,22133185
x1,114:12245612,22133185
x1,114:12671455,22133185
x1,114:13589209,22133185
k1,114:13933617,22133185:344408
x1,114:14424938,22133185
k1,114:14769346,22133185:344408
x1,114:15490101,22133185
k1,114:15834508,22133185:344407
x1,114:16325829,22133185
x1,114:17374530,22133185
k1,114:17718938,22133185:344408
x1,114:18570640,22133185
x1,114:18767049,22133185
k1,118:18767049,22133185:0
)
(1,118:3923141,22854081:14843908,406386,127692
x1,118:4447480,22854081
x1,118:4742392,22854081
x1,118:5025510,22854081
x1,118:5943264,22854081
k1,114:6290505,22854081:347241
x1,114:6749382,22854081
k1,114:7096623,22854081:347241
x1,114:7817378,22854081
k1,114:8164620,22854081:347242
x1,114:9114219,22854081
x1,114:10064417,22854081
k1,114:10411658,22854081:347241
x1,114:10902979,22854081
x1,114:11197891,22854081
k1,114:11545132,22854081:347241
x1,114:12004009,22854081
k1,114:12351250,22854081:347241
x1,114:13710789,22854081
k1,114:14058030,22854081:347241
x1,114:14680880,22854081
k1,115:14058030,22854081:-2946
x1,115:15349737,22854081
k1,115:15696979,22854081:347242
x1,115:16794624,22854081
k1,115:17141865,22854081:347241
x1,115:17535273,22854081
k1,115:17882313,22854081:347040
x1,115:18767049,22854081
k1,118:18767049,22854081:0
)
(1,118:3923141,23574977:14843908,402253,127692
x1,118:5643063,23574977
k1,115:6218380,23574977:575317
x1,115:7250572,23574977
k1,115:7825888,23574977:575316
x1,115:10857538,23574977
k1,116:7825888,23574977:-10613
x1,116:14287940,23574977
x1,116:15694061,23574977
x1,116:18767049,23574977
k1,116:18767049,23574977:0
)
(1,118:3923141,24295873:14843908,402253,127692
x1,118:5167653,24295873
x1,117:8413448,24295873
g1,117:8560904,24295873
x1,117:9805424,24295873
x1,117:10935522,24295873
k1,118:18767049,24295873:7831527
g1,118:18767049,24295873
)
(1,125:3923141,25158763:14843908,402253,127692
(1,119:3923141,25158763:0,380108,6778
g1,119:3923141,25158763
g1,119:3169481,25158763
g1,119:2841801,25158763
(1,119:2841801,25158763:753660,380108,6778
k1,119:3144903,25158763:303102
$1,119:3144903,25158763
x1,119:3448005,25158763
$1,119:3448005,25158763
x1,119:3595461,25158763
)
g1,119:3923141,25158763
)
x1,119:4283522,25158763
k1,120:3923141,25158763:-43647
x1,120:4387331,25158763
k1,120:4771537,25158763:384206
x1,120:5492300,25158763
x1,120:6911403,25158763
k1,120:7354795,25158763:443392
x1,120:7715176,25158763
x1,120:7818985,25158763
k1,120:8203191,25158763:384206
x1,120:8793007,25158763
x1,120:10496986,25158763
k1,120:10881192,25158763:384206
x1,120:11732894,25158763
k1,120:12117100,25158763:384206
x1,120:12788903,25158763
k1,120:13173109,25158763:384206
x1,120:14057837,25158763
k1,120:14442042,25158763:384205
x1,120:14835450,25158763
x1,120:15097328,25158763
x1,120:16327684,25158763
k1,121:16711890,25158763:384206
x1,121:17563592,25158763
k1,121:17947798,25158763:384206
x1,121:18570640,25158763
x1,121:18767049,25158763
k1,125:18767049,25158763:0
)
(1,125:3923141,25879659:14843908,402253,127692
x1,125:4709374,25879659
x1,125:4995444,25879659
x1,125:5543392,25879659
k1,121:6007363,25879659:463971
x1,121:6302275,25879659
x1,121:7270162,25879659
k1,121:7734132,25879659:463970
x1,121:8225453,25879659
k1,121:8689423,25879659:463970
x1,121:9410178,25879659
k1,121:9874149,25879659:463971
x1,121:11086232,25879659
k1,121:11549884,25879659:463652
x1,121:12925925,25879659
x1,121:14170445,25879659
k1,121:14634416,25879659:463971
x1,121:15584015,25879659
x1,121:16534213,25879659
k1,121:16998183,25879659:463970
x1,121:18570640,25879659
x1,121:18767049,25879659
k1,125:18767049,25879659:0
)
(1,125:3923141,26600555:14843908,406386,127692
x1,125:4906365,26600555
k1,121:5538505,26600555:632140
x1,121:6554172,26600555
x1,121:7700770,26600555
k1,121:8332910,26600555:632140
x1,121:9086699,26600555
x1,121:10413787,26600555
k1,121:11167097,26600555:753310
x1,121:11789947,26600555
k1,122:11167097,26600555:-2946
x1,122:12458804,26600555
k1,122:13090944,26600555:632140
x1,122:13746230,26600555
x1,122:14026396,26600555
x1,122:14135519,26600555
k1,122:14767659,26600555:632140
x1,122:15193510,26600555
k1,122:15825163,26600555:631653
x1,122:16414987,26600555
k1,122:17047127,26600555:632140
x1,122:18767049,26600555
k1,122:18767049,26600555:0
)
(1,125:3923141,27321451:14843908,402253,127692
x1,125:5840069,27321451
k1,122:8046480,27321451:2206411
x1,122:11078130,27321451
k1,123:8046480,27321451:-10613
x1,123:14230137,27321451
x1,123:15406824,27321451
x1,123:18767049,27321451
k1,123:18767049,27321451:0
)
(1,125:3923141,28042347:14843908,402253,127692
x1,125:5167653,28042347
x1,124:8413448,28042347
g1,124:8560904,28042347
x1,124:9805424,28042347
x1,124:10935522,28042347
k1,125:18767049,28042347:7831527
g1,125:18767049,28042347
)
(1,132:3923141,28905238:14843908,402253,127692
(1,126:3923141,28905238:0,380108,6778
g1,126:3923141,28905238
g1,126:3169481,28905238
g1,126:2841801,28905238
(1,126:2841801,28905238:753660,380108,6778
k1,126:3144903,28905238:303102
$1,126:3144903,28905238
x1,126:3448005,28905238
$1,126:3448005,28905238
x1,126:3595461,28905238
)
g1,126:3923141,28905238
)
x1,126:4398535,28905238
k1,127:4876518,28905238:477983
x1,127:5302369,28905238
x1,127:5980075,28905238
x1,127:6269089,28905238
x1,127:6555159,28905238
x1,127:6664282,28905238
k1,127:7224897,28905238:560615
x1,127:8044148,28905238
x1,127:8600938,28905238
x1,127:9190746,28905238
x1,127:9944535,28905238
k1,128:10422518,28905238:477983
x1,128:11143273,28905238
k1,128:11621257,28905238:477984
x1,128:11949195,28905238
x1,128:12229361,28905238
x1,128:12678806,28905238
x1,128:13727507,28905238
k1,128:14205490,28905238:477983
x1,128:15417573,28905238
k1,128:15895224,28905238:477651
x1,128:16746926,28905238
x1,128:17271265,28905238
x1,128:17566177,28905238
x1,128:17849295,28905238
x1,128:18767049,28905238
k1,128:18767049,28905238:0
)
(1,132:3923141,29626134:14843908,402253,127692
x1,132:4382018,29626134
k1,128:4861706,29626134:479688
x1,128:5582461,29626134
k1,128:6062150,29626134:479689
x1,128:7011749,29626134
x1,128:7961947,29626134
k1,128:8441635,29626134:479688
x1,128:10014092,29626134
x1,128:10997316,29626134
k1,128:11477004,29626134:479688
x1,128:12492671,29626134
x1,128:13639269,29626134
k1,128:14118957,29626134:479688
x1,128:14872746,29626134
x1,128:16216343,29626134
k1,128:17063652,29626134:847309
x1,128:18767049,29626134
k1,128:18767049,29626134:0
)
(1,132:3923141,30347030:14843908,406386,127692
x1,132:4971834,30347030
x1,132:5725623,30347030
k1,128:6183742,30347030:458119
x1,128:6904497,30347030
x1,128:7658286,30347030
k1,128:8116406,30347030:458120
x1,128:9541998,30347030
k1,128:10077782,30347030:535784
x1,128:10700632,30347030
k1,129:10077782,30347030:-2946
x1,129:11369489,30347030
k1,129:11827608,30347030:458119
x1,129:12482894,30347030
x1,129:12763060,30347030
x1,129:12872183,30347030
k1,129:13330303,30347030:458120
x1,129:13756154,30347030
k1,129:14213960,30347030:457806
x1,129:15098696,30347030
k1,129:15556816,30347030:458120
x1,129:17129282,30347030
k1,129:17587401,30347030:458119
x1,129:18767049,30347030
k1,129:18767049,30347030:0
)
(1,132:3923141,31067926:14843908,402253,127692
x1,132:5692613,31067926
k1,129:7751568,31067926:2058955
x1,129:10783218,31067926
k1,130:7751568,31067926:-10613
x1,130:13935225,31067926
x1,130:15111912,31067926
x1,130:18767049,31067926
k1,130:18767049,31067926:0
)
(1,132:3923141,31788822:14843908,402253,127692
x1,132:5167653,31788822
x1,131:8413448,31788822
g1,131:8560904,31788822
x1,131:9805424,31788822
x1,131:10935522,31788822
k1,132:18767049,31788822:7831527
g1,132:18767049,31788822
)
]
k1,161:19356873,31788822:589824
r1,163:19356873,31788822:0,19671608,141880
k1,161:19946697,31788822:589824
[1,161:19946697,31788822:15925248,19529728,127692
(1,139:21028037,12914454:14843908,402253,127692
(1,133:21028037,12914454:0,380108,6778
g1,133:21028037,12914454
g1,133:20274377,12914454
g1,133:19946697,12914454
(1,133:19946697,12914454:753660,380108,6778
k1,133:20249799,12914454:303102
$1,133:20249799,12914454
x1,133:20552901,12914454
$1,133:20552901,12914454
x1,133:20700357,12914454
)
g1,133:21028037,12914454
)
x1,133:21535874,12914454
k1,134:21962340,12914454:426466
x1,134:23256403,12914454
k1,134:23752621,12914454:496218
x1,134:24325928,12914454
k1,134:24752395,12914454:426467
x1,134:25293259,12914454
k1,134:25719725,12914454:426466
x1,134:26735400,12914454
x1,134:27488599,12914454
k1,134:27915065,12914454:426466
x1,134:28766767,12914454
k1,134:29193234,12914454:426467
x1,134:29553615,12914454
x1,134:29657424,12914454
k1,134:30083890,12914454:426466
x1,134:30870705,12914454
x1,134:32295706,12914454
k1,134:32791924,12914454:496218
x1,134:34430434,12914454
x1,134:35871945,12914454
k1,135:35871945,12914454:0
)
(1,139:21028037,13635350:14843908,406386,127692
x1,139:22273139,13635350
x1,139:23092398,13635350
k1,135:23634713,13635350:542315
x1,135:24093590,13635350
k1,135:24635905,13635350:542315
x1,135:25225721,13635350
x1,135:25881007,13635350
x1,135:26634206,13635350
x1,135:26962136,13635350
x1,135:27242302,13635350
x1,135:27495338,13635350
k1,135:28037653,13635350:542315
x1,135:28921791,13635350
x1,135:29204909,13635350
x1,135:29827751,13635350
x1,135:29936874,13635350
k1,135:30577902,13635350:641028
x1,135:31200752,13635350
k1,136:30577902,13635350:-2946
x1,136:31869609,13635350
k1,136:32411924,13635350:542315
x1,136:33509569,13635350
k1,136:34051884,13635350:542315
x1,136:34445292,13635350
k1,136:34987209,13635350:541917
x1,136:35871945,13635350
k1,139:35871945,13635350:0
)
(1,139:21028037,14356246:14843908,402253,127692
x1,139:22747959,14356246
k1,136:23408794,14356246:660835
x1,136:24440986,14356246
k1,136:25101822,14356246:660836
x1,136:28133472,14356246
k1,137:25101822,14356246:-10613
x1,137:32038686,14356246
x1,137:35871945,14356246
k1,139:35871945,14356246:0
)
(1,139:21028037,15077142:14843908,402253,127692
x1,139:21584827,15077142
g1,137:21732283,15077142
x1,137:22976795,15077142
k1,138:21732283,15077142:-14746
x1,138:25485310,15077142
g1,138:25632766,15077142
x1,138:26877286,15077142
x1,138:28007384,15077142
k1,139:35871945,15077142:7864561
g1,139:35871945,15077142
)
(1,145:21028037,16072098:14843908,402253,127692
h1,140:21028037,16072098:0,0,0
x1,140:21535874,16072098
k1,140:21962340,16072098:426466
x1,140:23256403,16072098
k1,140:23752621,16072098:496218
x1,140:24325928,16072098
k1,140:24752395,16072098:426467
x1,140:25293259,16072098
k1,140:25719725,16072098:426466
x1,140:26735400,16072098
x1,140:27488599,16072098
k1,140:27915065,16072098:426466
x1,140:28766767,16072098
k1,140:29193234,16072098:426467
x1,140:29553615,16072098
x1,140:29657424,16072098
k1,140:30083890,16072098:426466
x1,140:30870705,16072098
x1,140:32295706,16072098
k1,140:32791924,16072098:496218
x1,140:34430434,16072098
x1,140:35871945,16072098
k1,141:35871945,16072098:0
)
(1,145:21028037,16792994:14843908,406386,127692
x1,145:22273139,16792994
x1,145:23092398,16792994
k1,141:23634713,16792994:542315
x1,141:24093590,16792994
k1,141:24635905,16792994:542315
x1,141:25225721,16792994
x1,141:25881007,16792994
x1,141:26634206,16792994
x1,141:26962136,16792994
x1,141:27242302,16792994
x1,141:27495338,16792994
k1,141:28037653,16792994:542315
x1,141:28921791,16792994
x1,141:29204909,16792994
x1,141:29827751,16792994
x1,141:29936874,16792994
k1,141:30577902,16792994:641028
x1,141:31200752,16792994
k1,142:30577902,16792994:-2946
x1,142:31869609,16792994
k1,142:32411924,16792994:542315
x1,142:33509569,16792994
k1,142:34051884,16792994:542315
x1,142:34445292,16792994
k1,142:34987209,16792994:541917
x1,142:35871945,16792994
k1,145:35871945,16792994:0
)
(1,145:21028037,17513890:14843908,402253,127692
x1,145:22747959,17513890
k1,142:23408794,17513890:660835
x1,142:24440986,17513890
k1,142:25101822,17513890:660836
x1,142:28133472,17513890
k1,143:25101822,17513890:-10613
x1,143:32038686,17513890
x1,143:35871945,17513890
k1,145:35871945,17513890:0
)
(1,145:21028037,18234786:14843908,402253,127692
x1,145:21584827,18234786
g1,143:21732283,18234786
x1,143:22976795,18234786
k1,144:21732283,18234786:-14746
x1,144:25485310,18234786
g1,144:25632766,18234786
x1,144:26877286,18234786
x1,144:28007384,18234786
k1,145:35871945,18234786:7864561
g1,145:35871945,18234786
)
(1,148:21028037,19503801:14843908,402253,127692
(1,146:21028037,19503801:0,380108,6778
g1,146:21028037,19503801
g1,146:20274377,19503801
g1,146:19946697,19503801
(1,146:19946697,19503801:753660,380108,6778
k1,146:20249799,19503801:303102
$1,146:20249799,19503801
x1,146:20552901,19503801
$1,146:20552901,19503801
x1,146:20700357,19503801
)
g1,146:21028037,19503801
)
x1,146:21535874,19503801
k1,147:21709400,19503801:173526
x1,147:22856007,19503801
k1,147:23029532,19503801:173525
x1,147:23881234,19503801
k1,147:24054760,19503801:173526
x1,147:24628067,19503801
k1,147:24801592,19503801:173525
x1,147:25374899,19503801
k1,147:25548425,19503801:173526
x1,147:25974276,19503801
x1,147:26772892,19503801
x1,147:27642284,19503801
x1,147:27766152,19503801
k1,147:27946194,19503801:180042
x1,147:29289800,19503801
k1,147:29463326,19503801:173526
x1,147:30020116,19503801
x1,147:31035783,19503801
x1,147:31625607,19503801
x1,147:32019007,19503801
x1,147:32936761,19503801
k1,147:33110286,19503801:173525
x1,147:33601607,19503801
k1,147:33775133,19503801:173526
x1,147:34823244,19503801
x1,147:35871945,19503801
k1,147:35871945,19503801:0
)
(1,148:21028037,20224697:14843908,406386,127692
x1,148:21748792,20224697
x1,148:22371634,20224697
x1,148:23616736,20224697
k1,147:23778339,20224697:161603
x1,147:24237216,20224697
k1,147:24398819,20224697:161603
x1,147:24693731,20224697
x1,147:25804365,20224697
k1,147:25965968,20224697:161603
x1,147:26686723,20224697
x1,147:26981635,20224697
x1,147:27980778,20224697
k1,147:28145918,20224697:165140
x1,147:29439980,20224697
k1,147:29601583,20224697:161603
x1,147:30224433,20224697
x1,147:30893290,20224697
k1,147:31054893,20224697:161603
x1,147:31595757,20224697
k1,147:31757360,20224697:161603
x1,147:32789552,20224697
k1,147:32954691,20224697:165139
x1,147:34674613,20224697
k1,147:34839753,20224697:165140
x1,147:35871945,20224697
k1,147:35871945,20224697:0
)
(1,148:21028037,20945593:14843908,402253,127692
x1,148:24059687,20945593
x1,147:27964901,20945593
x1,147:31798160,20945593
x1,147:32371467,20945593
k1,148:35871945,20945593:3500478
g1,148:35871945,20945593
)
(1,151:21028037,22214608:14843908,402253,127692
(1,149:21028037,22214608:0,380108,6778
g1,149:21028037,22214608
g1,149:20274377,22214608
g1,149:19946697,22214608
(1,149:19946697,22214608:753660,380108,6778
g1,149:19946697,22214608
$1,149:19946697,22214608
x1,149:20552901,22214608
$1,149:20552901,22214608
x1,149:20700357,22214608
)
g1,149:21028037,22214608
)
x1,149:21535874,22214608
k1,150:21798005,22214608:262131
x1,150:22944612,22214608
k1,150:23206743,22214608:262131
x1,150:24058445,22214608
k1,150:24320575,22214608:262130
x1,150:24893882,22214608
k1,150:25156013,22214608:262131
x1,150:25729320,22214608
k1,150:25991451,22214608:262131
x1,150:26417302,22214608
x1,150:27215918,22214608
x1,150:28085310,22214608
x1,150:28209178,22214608
k1,150:28499977,22214608:290799
x1,150:29417148,22214608
k1,150:29679279,22214608:262131
x1,150:30694946,22214608
x1,150:31284770,22214608
x1,150:31710613,22214608
x1,150:32628367,22214608
k1,150:32890497,22214608:262130
x1,150:33381818,22214608
k1,150:33643949,22214608:262131
x1,150:34692650,22214608
k1,150:34954781,22214608:262131
x1,150:35675536,22214608
x1,150:35871945,22214608
k1,151:35871945,22214608:0
)
(1,151:21028037,22935504:14843908,406386,127692
x1,151:21650879,22935504
x1,151:22895981,22935504
k1,150:23179171,22935504:283190
x1,150:23638048,22935504
k1,150:23921238,22935504:283190
x1,150:24216150,22935504
x1,150:25326784,22935504
k1,150:25609973,22935504:283189
x1,150:26330728,22935504
x1,150:26625640,22935504
x1,150:27624783,22935504
k1,150:27941906,22935504:317123
x1,150:29235968,22935504
k1,150:29519158,22935504:283190
x1,150:30142008,22935504
x1,150:30810865,22935504
k1,150:31094055,22935504:283190
x1,150:31487463,22935504
k1,150:31770516,22935504:283053
x1,150:34522630,22935504
k1,150:34839753,22935504:317123
x1,150:35871945,22935504
k1,150:35871945,22935504:0
)
(1,151:21028037,23656400:14843908,402253,127692
x1,151:24059687,23656400
x1,150:27964901,23656400
x1,150:31798160,23656400
x1,150:32354950,23656400
x1,150:32448146,23656400
k1,151:35871945,23656400:3423799
g1,151:35871945,23656400
)
(1,154:21028037,24925416:14843908,402253,127692
(1,152:21028037,24925416:0,380108,6778
g1,152:21028037,24925416
g1,152:20274377,24925416
g1,152:19946697,24925416
(1,152:19946697,24925416:753660,380108,6778
g1,152:19946697,24925416
$1,152:19946697,24925416
x1,152:20552901,24925416
$1,152:20552901,24925416
x1,152:20700357,24925416
)
g1,152:21028037,24925416
)
x1,152:21699840,24925416
k1,153:22064264,24925416:364424
x1,153:22441155,24925416
k1,153:22805579,24925416:364424
x1,153:24836891,24925416
x1,153:24960759,24925416
k1,153:25379425,24925416:418666
x1,153:26592083,24925416
k1,153:26956507,24925416:364424
x1,153:27677262,24925416
x1,153:28463495,24925416
k1,153:28827919,24925416:364424
x1,153:29876612,24925416
x1,153:30630401,24925416
k1,153:30994825,24925416:364424
x1,153:31584641,24925416
x1,153:32165623,24925416
x1,153:33181290,24925416
k1,153:33545714,24925416:364424
x1,153:34004591,24925416
x1,153:34266469,24925416
x1,153:35871945,24925416
k1,153:35871945,24925416:0
)
(1,154:21028037,25646312:14843908,406386,127692
x1,154:22010678,25646312
k1,153:22261527,25646312:250849
x1,153:23310228,25646312
k1,153:23561078,25646312:250850
x1,153:23822956,25646312
x1,153:24724784,25646312
x1,153:25052714,25646312
x1,153:25332880,25646312
x1,153:25585916,25646312
k1,153:25836765,25646312:250849
x1,153:26360521,25646312
x1,153:27655166,25646312
k1,153:27931864,25646312:276698
x1,153:29225926,25646312
k1,153:29476776,25646312:250850
x1,153:30099626,25646312
x1,153:30768483,25646312
k1,153:31019332,25646312:250849
x1,153:31412740,25646312
k1,153:31663485,25646312:250745
x1,153:34563055,25646312
k1,153:34839753,25646312:276698
x1,153:35871945,25646312
k1,153:35871945,25646312:0
)
(1,154:21028037,26367208:14843908,402253,127692
x1,154:24059687,26367208
x1,153:27964901,26367208
x1,153:31798160,26367208
x1,153:32224011,26367208
x1,153:32442840,26367208
k1,154:35871945,26367208:3429105
g1,154:35871945,26367208
)
(1,157:21028037,27636223:14843908,402253,127692
(1,155:21028037,27636223:0,380108,6778
g1,155:21028037,27636223
g1,155:20274377,27636223
g1,155:19946697,27636223
(1,155:19946697,27636223:753660,380108,6778
g1,155:19946697,27636223
$1,155:19946697,27636223
x1,155:20552901,27636223
$1,155:20552901,27636223
x1,155:20700357,27636223
)
g1,155:21028037,27636223
)
x1,155:21568901,27636223
k1,156:21849934,27636223:281033
x1,156:22177872,27636223
x1,156:22259858,27636223
k1,156:22540892,27636223:281034
x1,156:23130708,27636223
x1,156:23711690,27636223
x1,156:24874813,27636223
k1,156:25189240,27636223:314427
x1,156:26434342,27636223
x1,156:26696220,27636223
x1,156:27580940,27636223
x1,156:27744905,27636223
x1,156:28432626,27636223
k1,156:28713659,27636223:281033
x1,156:29041597,27636223
x1,156:29327667,27636223
x1,156:30277865,27636223
x1,156:30703708,27636223
x1,156:31621462,27636223
k1,156:31902495,27636223:281033
x1,156:32393816,27636223
k1,156:32674850,27636223:281034
x1,156:33395605,27636223
k1,156:33676638,27636223:281033
x1,156:34954191,27636223
x1,156:35871945,27636223
k1,156:35871945,27636223:0
)
(1,157:21028037,28357119:14843908,406386,127692
x1,157:21945208,28357119
x1,157:22731441,28357119
k1,156:22912939,28357119:181498
x1,156:23404260,28357119
k1,156:23585758,28357119:181498
x1,156:24633860,28357119
x1,156:25289146,28357119
x1,156:26304813,28357119
x1,156:27451411,28357119
k1,156:27632909,28357119:181498
x1,156:28124230,28357119
x1,156:28550073,28357119
x1,156:29270238,28357119
x1,156:30335448,28357119
k1,156:30525457,28357119:190009
x1,156:31148307,28357119
x1,156:31817164,28357119
k1,156:31998662,28357119:181498
x1,156:32653948,28357119
x1,156:32934114,28357119
x1,156:33043237,28357119
k1,156:33224735,28357119:181498
x1,156:33962015,28357119
k1,156:34152023,28357119:190008
x1,156:35871945,28357119
k1,156:35871945,28357119:0
)
(1,157:21028037,29078015:14843908,402253,127692
x1,157:22060229,29078015
g1,156:22207685,29078015
x1,156:26336981,29078015
x1,156:30406742,29078015
x1,156:31583429,29078015
x1,156:31863595,29078015
x1,156:33742190,29078015
k1,157:35871945,29078015:2129755
g1,157:35871945,29078015
)
(1,160:21028037,30347030:14843908,402253,127692
(1,158:21028037,30347030:0,380108,6778
g1,158:21028037,30347030
g1,158:20274377,30347030
g1,158:19946697,30347030
(1,158:19946697,30347030:753660,380108,6778
g1,158:19946697,30347030
$1,158:19946697,30347030
x1,158:20552901,30347030
$1,158:20552901,30347030
x1,158:20700357,30347030
)
g1,158:21028037,30347030
)
x1,158:21896839,30347030
k1,159:21028037,30347030:-65470
x1,159:21978825,30347030
k1,159:22294913,30347030:316088
x1,159:22884729,30347030
x1,159:23465711,30347030
x1,159:24628834,30347030
k1,159:24987079,30347030:358245
x1,159:25707842,30347030
k1,159:26023929,30347030:316087
x1,159:26744692,30347030
x1,159:27006570,30347030
x1,159:27464857,30347030
x1,159:28120143,30347030
k1,159:28436231,30347030:316088
x1,159:29255482,30347030
x1,159:29812272,30347030
x1,159:30500584,30347030
k1,159:30816671,30347030:316087
x1,159:31504400,30347030
x1,159:31787518,30347030
x1,159:32541307,30347030
k1,159:32857395,30347030:316088
x1,159:33578158,30347030
x1,159:34201000,30347030
x1,159:34724756,30347030
x1,159:35871945,30347030
k1,159:35871945,30347030:0
)
(1,160:21028037,31067926:14843908,406386,127692
x1,160:21486914,31067926
k1,159:21791821,31067926:304907
x1,159:23069374,31067926
x1,159:23987128,31067926
k1,159:24292035,31067926:304907
x1,159:25340137,31067926
x1,159:25995423,31067926
x1,159:26585247,31067926
x1,159:27600914,31067926
x1,159:28403648,31067926
k1,159:28747917,31067926:344269
x1,159:29370767,31067926
x1,159:30039624,31067926
k1,159:30344531,31067926:304907
x1,159:30999817,31067926
x1,159:31279983,31067926
x1,159:31389106,31067926
k1,159:31694013,31067926:304907
x1,159:32431293,31067926
k1,159:32775562,31067926:344269
x1,159:34495484,31067926
k1,159:34839753,31067926:344269
x1,159:35871945,31067926
k1,159:35871945,31067926:0
)
(1,160:21028037,31788822:14843908,402253,127692
x1,160:25157333,31788822
x1,159:29227094,31788822
x1,159:30403781,31788822
x1,159:30683947,31788822
x1,159:32562542,31788822
k1,160:35871945,31788822:3309403
g1,160:35871945,31788822
)
]
(1,161:35871945,31788822:0,298188,141880
h1,161:35871945,31788822:327680,298188,141880
k1,161:35871945,31788822:-327680
)
)
]
(1,163:2841801,49947279:33030144,406386,104688
(1,163:2841801,49947279:33030144,406386,104688
g1,163:2841801,49947279
(1,163:2841801,49947279:33030144,406386,104688
k1,163:14788726,49947279:11946925
x1,163:15410985,49947279
x1,163:15664021,49947279
x1,163:15767830,49947279
g1,163:15915286,49947279
x1,163:16668485,49947279
x1,163:17066025,49947279
g1,163:17213481,49947279
x1,163:17573862,49947279
x1,163:18088178,49947279
g1,163:18271022,49947279
x1,163:18860846,49947279
g1,163:19043690,49947279
x1,163:20288210,49947279
g1,163:20435666,49947279
x1,163:21875996,49947279
g1,163:22058840,49947279
x1,163:22844474,49947279
x1,163:23925020,49947279
k1,163:35871945,49947279:11946925
)
g1,163:35871945,49947279
)
)
]
]
!50244
}2
Input:33:C:\Users\eddy_\Dropbox\University\Mexico\Presentations\2021 08 DPyC\Proceedings\Plantilla-rmf\Research-Education-ingles.aux
!143
Postamble:
Count:2262
!27
Post scriptum:

